Drift and Meander of Spiral Waves

In this thesis, we are concerned with the dynamics of spiral wave solutions to Reaction-Diffsion systems of equations, and how they behave when subject to symmetry breaking perturbations. We present an asymptotic theory of the study of meandering (quasiperiodic spiral wave solutions) spiral waves which are drifting due to symmetry breaking perturbations. This theory is based on earlier theories: the 1995 Biktashev et al theory of drift of rigidly rotating spirals, and the 1996 Biktashev et al theory of meander of spirals in unperturbed systems. We combine the two theories by first rewriting the 1995 drift theory using the symmetry quotient system method of the 1996 meander theory, and then go on to extend the approach to meandering spirals by considering Floquet theory and using a singular perturbation method. We demonstrate the work of the newly developed theory on simple examples. We also develop a numerical implementation of the quotient system method, demonstrate its numerical convergence and its use in calculations which would be difficult to do by the standard methods, and also link this study to the problem of calculation of response functions of spiral waves.

==> chapter1/defs.tex <==
\newtheorem{thm}{Theorem}[section]

\theoremstyle{definition}	

\newtheorem{defn}[thm]{Definition}

\newcommand{\ez}{EZ-Freeze }

%%%%%%%%%%%%%%%%% Group Actions etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dd}{\textrm{d}}
\newcommand{\dT}{\textrm{T}(g)}
\newcommand{\ddT}{\textrm{T}(dg)}
\newcommand{\dTddT}{\textrm{T}(g+dg)}
\newcommand{\dTi}{\textrm{T}(g^{-1})}
\newcommand{\ddTi}{\textrm{T}(dg^{-1})}
\newcommand{\ddTcom}{\textrm{T}(\{\textbf{c}dt,\omega dt\})}

%%%%%%%%%%%%%%%%% Bold letters and Symbols %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Greek

\newcommand{\balp}{\boldsymbol{\alpha}}
\newcommand{\bbet}{\boldsymbol{\beta}}
\newcommand{\bet}{\boldsymbol{\eta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

%Latin

\newcommand{\bA}{\textbf{A}}
\newcommand{\bD}{\textbf{B}}
\newcommand{\bc}{\textbf{c}}
\newcommand{\bC}{\textbf{C}}
\newcommand{\be}{\textbf{e}}
\newcommand{\bof}{\textbf{f}}
\newcommand{\boof}{\textbf{f}}
\newcommand{\booF}{\textbf{F}}
\newcommand{\boF}{\textbf{F}(\textbf{V})}
\newcommand{\boFU}{\textbf{F}(\textbf{U})}
\newcommand{\boFt}{\textbf{F}(\textbf{t})}
\newcommand{\bFg}{\textbf{F}_{\mathcal{G}}(\bV)}
\newcommand{\bFm}{\textbf{F}_{\mathcal{M}}(\bV)}
\newcommand{\bg}{\textbf{g}}
\newcommand{\bG}{\textbf{G}}
\newcommand{\bGt}{\textbf{G}(\textbf{t})}
\newcommand{\bh}{\textbf{h}}
\newcommand{\bH}{\textbf{H}}
\newcommand{\bHg}{\til{\bH}_{\mathcal{G}}(\bV,t)}
\newcommand{\bHm}{\til{\bH}_{\mathcal{M}}(\bV,t)}
\newcommand{\bI}{\textbf{I}}
\newcommand{\bk}{\textbf{k}}
\newcommand{\bM}{\textbf{M}}
\newcommand{\bP}{\textbf{P}}
\newcommand{\bp}{\textbf{p}}
\newcommand{\bq}{\textbf{q}}
\newcommand{\bQ}{\textbf{Q}}
\newcommand{\br}{\textbf{r}}
\newcommand{\bR}{\textbf{R}}
\newcommand{\bS}{\textbf{S}}
\newcommand{\bu}{\textbf{u}}
\newcommand{\bU}{\textbf{U}}
\newcommand{\bv}{\textbf{v}}
\newcommand{\bV}{\textbf{V}}
\newcommand{\bw}{\textbf{w}}
\newcommand{\bW}{\textbf{W}}

%%%%%%%%%%%%%%%%% letters with hats and tildes %%%%%%%%%%%%%%%%%

\newcommand{\til}{\tilde}
\newcommand{\bDh}{\hat{\textbf{D}}}
\newcommand{\Bh}{\hat{\partial}}
\newcommand{\hh}{\hat{\textbf{h}}}
\newcommand{\bHt}{\tilde{\textbf{H}}(\textbf{V},t)}
\newcommand{\tH}{\tilde{\textbf{H}}}
\newcommand{\bht}{\tilde{\textbf{h}}}
\newcommand{\btr}{\tilde{\textbf{r}}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tr}{\tilde{r}}
\newcommand{\tbr}{\tilde{\textbf{r}}}
\newcommand{\ttim}{\tilde{t}}
\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tth}{\tilde{\theta}}

%%%%%%%%%%%%%%%%% Derivatives %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\deriv}[2]{\frac{\dd #1}{\dd #2}}

%ODE's

\newcommand{\odcxot}{\frac{\dd{\bc_{x0}}}{\dd{t}}}
\newcommand{\odcyot}{\frac{\dd{\bc_{y0}}}{\dd{t}}}
\newcommand{\odcot}{\frac{\dd{\bc_0}}{\dd{t}}}
\newcommand{\odomt}{\frac{\dd{\omega}}{\dd{t}}}
\newcommand{\odRt}{\frac{\dd{R}}{\dd{t}}}
\newcommand{\odbRt}{\frac{\dd{\bR}}{\dd{t}}}
\newcommand{\odTt}{\frac{\dd{\dT}}{\dd{t}}}
\newcommand{\odTht}{\frac{\dd{\Theta}}{\dd{t}}}
\newcommand{\odThot}{\frac{\dd{\Theta_0}}{\dd{t}}}
\newcommand{\odThonet}{\frac{\dd{\Theta_1}}{\dd{t}}}
\newcommand{\odbut}{\frac{\dd{\bu}}{\dd{t}}}
\newcommand{\odbUt}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odut}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odbvt}{\frac{\dd{\bv}}{\dd{t}}}
\newcommand{\odbVt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbVot}{\frac{\dd{\bV_0}}{\dd{t}}}
\newcommand{\odbVpt}{\frac{\dd{\bV_1}}{\dd{t}}}
\newcommand{\odvt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbvpit}{\frac{\dd{\bv}_{pi}}{\dd{t}}}
\newcommand{\odbVpit}{\frac{\dd{\bV}_{1pi}}{\dd{t}}}
\newcommand{\odbwt}{\frac{\dd{\bw}}{\dd{t}}}
\newcommand{\odbWt}{\frac{\dd{\bW}}{\dd{t}}}
\newcommand{\odXt}{\frac{\dd{X}}{\dd{t}}}
\newcommand{\odYt}{\frac{\dd{Y}}{\dd{t}}}

%PDE's - wrt x

\newcommand{\pdbvx}{\frac{\partial{\textbf{v}}}{\partial{x}}}
\newcommand{\pdbux}{\frac{\partial{\textbf{u}}}{\partial{x}}}
\newcommand{\pdux}{\frac{\partial{u}}{\partial{x}}}
\newcommand{\pdvx}{\frac{\partial{v}}{\partial{x}}}
\newcommand{\pdvxk}{\frac{\partial{v^{(i)}_k}}{\partial{x}}}
\newcommand{\pduox}{\frac{\partial{\textbf{u}_0}}{\partial{x}}}
\newcommand{\pdvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbtvox}{\frac{\partial{\til{\textbf{v}}_0}}{\partial{x}}}
\newcommand{\pdvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{x}}}}
\newcommand{\pdbvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\til{x}}}}
\newcommand{\pdvoxx}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}^2}}
\newcommand{\pdtrtx}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{x}}}}
\newcommand{\pdtthtx}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{x}}}}
\newcommand{\pdtxx}{\frac{\partial{\tilde{x}}}{\partial{x}}}
\newcommand{\pdtyx}{\frac{\partial{\tilde{y}}}{\partial{x}}}
\newcommand{\pdax}{\frac{\partial{\alpha}}{\partial{x}}}

%PDE's - wrt y

\newcommand{\pdbvy}{\frac{\partial{\textbf{v}}}{\partial{y}}}
\newcommand{\pduoy}{\frac{\partial{\textbf{u}_0}}{\partial{y}}}
\newcommand{\pdvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\til{y}}}}
\newcommand{\pdvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{y}}}}
\newcommand{\pdvoyy}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}^2}}
\newcommand{\pdtrty}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{y}}}}
\newcommand{\pdtthty}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{y}}}}
\newcommand{\pdtxy}{\frac{\partial{\tilde{x}}}{\partial{y}}}
\newcommand{\pdtyy}{\frac{\partial{\tilde{y}}}{\partial{y}}}

%PDE's - wrt theta

\newcommand{\pdbvth}{\frac{\partial{\textbf{v}}}{\partial{\theta}}}
\newcommand{\pdvoth}{\frac{\partial{\textbf{v}_0}}{\partial{\theta}}}
\newcommand{\pdvth}{\frac{\partial{\textbf{v}_1}}{\partial{\theta}}}
\newcommand{\pdvotth}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{\theta}}}}
\newcommand{\pdvothth}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}^2}}

%PDE's - wrt t

\newcommand{\pdvvtt}{\frac{\partial{\textbf{v}}_1}{\partial{\tilde{t}}}}
\newcommand{\pduot}{\frac{\partial{\textbf{u}_0}}{\partial{t}}}
\newcommand{\pdbut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvot}{\frac{\partial{\textbf{v}_0}}{\partial{t}}}
\newcommand{\pdvott}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{t}}}}
\newcommand{\pdtthtt}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{t}}}}
\newcommand{\pdut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvt}{\frac{\partial{\textbf{v}}}{\partial{t}}}

%PDE's - wrt u/v/U/V

\newcommand{\pdfa}{\frac{\partial{\textbf{f}}}{\partial{\alpha}}}
\newcommand{\pdfu}{\frac{\partial{\textbf{f}}}{\partial{\bu}}}
\newcommand{\pdfvov}{\frac{\partial{\textbf{f}(\textbf{v}_0)}}{\partial{\textbf{v}}}}
\newcommand{\pdgu}{\frac{\partial{\textbf{g}}}{\partial{\bV}}}

%PDE's mixed

\newcommand{\pdvoxy}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{y}}}
\newcommand{\pdvoxth}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{\theta}}}
\newcommand{\pdvoyx}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{x}}}
\newcommand{\pdvoyth}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{\theta}}}
\newcommand{\pdvothx}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{x}}}
\newcommand{\pdvothy}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{y}}}


==> chapter2/5_initial_analysis.tex <==
\section{Initial Numerical Analysis}

In this section we shall present some numerical analysis that was conducted during the author's first year of working on this project. We feel that although this is not original work and does not deserve a chapter to itself, it is rather interesting work and will hopefully expand the reader's knowledge of spiral wave behaviour.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Numerical Analysis of Spiral Waves that Drift due to Inhomogeneities}

\subsubsection{Introduction}
\label{ch:intro1}

In this chapter we study the drift of a spiral wave due to in homogeneities. We will firstly present the numerical work that we have carried out together with some preliminary results and conclusions, before providing an analytical approach to this particular area.

This project is primarily concerned with meandering spiral waves that drift due to inhomogeneities, but in order to get a feel of what drift due to inhomogeneities entails, we will look at rigid rotation before meander. EZSpiral is yet again used to help us in the numerical analysis of this particular area. When a wave drifts due to inhomogeneities (from now on I will simply say "drift" to mean "drift due to inhomogeneities"), it's parameters are dependant on the spatial coordinates. It's point of rotation is no longer stationary but drifts along a straight line. Therefore we have that $a=a(x,y)$.

We then adjusted the code to EZSpiral to take this dependency into account. Initally, we take $a=a_0+a_1x$ so that $a$ is linearly dependant on $x$ only. This now means that we have 4 parameters - $\epsilon,\ a_0,\ a_1,\ b$. Throughout this analysis we take $\epsilon=0.01$, as per previous work.


\subsubsection{Numerical Analysis}
\label{sec:numanal}

As mentioned in the introduction to this chapter, we are firstly going to look at rigid rotation (RW). Recall, that RW's are periodic solutions to the PDE system being studied. Their tips trace out a perfect circle. When viewed in a rotating frame of reference that rotates with a frequency equal to the frequency of the RW's, they appear to be stationary (a dot is abserved). This type of spiral is the simplest type of spiral to study from a Mathematical point of view and we will consider this firstly.

\subsection{Initial Analysis}

Using the parametric portrait obtained in the previous chapter, we chose $a_0,\ a_1,\ \&\ b$, such that we get a RW with a medium core radius. We therefore chose the following values:

\begin{eqnarray*}
a_0 & = & 0.7\\
a_1 & = & 0\\
b & = & 0.15\\
\epsilon & = & 0.01
\end{eqnarray*}

Other numerical and physical parameters were chosen as follows:

\begin{eqnarray*}
N_x & = & 181\\
L_x & = & 60\\
\mbox{Steps per plot} & = & 16\\
ts & = & 0.8
\end{eqnarray*}
\\
where $ts$ is timestep as a fraction of the diffusion stability limit. This means that our space step and time step were $h_x=\frac{1}{3}$ and $h_t=\frac{1}{30}$ respectively. These steps were kept constant throughout our analysis.

First of all we need to show that our amended EZSpiral ran correctly. We therefore ran the program for various values of $a_0$ with $a_1=0$. These runs were then compared to the original data using the original program. The results showed that the amended program gave exactly the same results as the original program. A couple of tests are shown below. Therefore, early indications show that the program is working correctly.

There is an established theory which states that for small gradients the speed of the wave is proportional to the gradient. Therefore, in order to test whether EZSpiral is certainly working correctly, we are to prove, numerically, this theory.

Firstly, we ran the program for a range of gradients, $a_1$. As usual, a \emph{tip.dat} file is produced from which we can extract a variety of information. We then calculated the "speed" of the wave using the tip file by plotting $t$ vs $x$ and $t$ vs $y$ using Gnuplot and made Gnuplot include a line of best fit. Several examples of these are included in figures \ref{fig:fitxy020} and \ref{fig:fitxy016}. The gradient of this line would then give me $\frac{dx}{dt}$ and $\frac{dy}{dt}$. Using $s=\sqrt{\dot{x}^2+\dot{y}^2}$, where $s$ is the speed of the wave and the "dots" represent the usual differentiation with respect to t, we then plotted $s$ vs gradient ($a_1$) and then observed what relationship(s), if any, are present.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx020.eps}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity020.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and $t$ vs $y$ on the right for $a_1=0.0005$}
\label{fig:fitxy020}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx016.eps}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity016.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and $t$ vs $y$ on the right for $a_1=0.0009$}
\label{fig:fitxy016}
\end{center}
\end{figure}

From the Gnuplot output and also using Maple to quickly calculate $s$, we get the following table of results:

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & s\\
\hline
-0.0038 & 0.111062 & -0.47453 & 0.487253\\
-0.00375 & 0.118094 & -0.513751 & 0.527149\\
-0.0035 & 0.150046	& -0.463961 & 0.487620\\
-0.003 & 0.0919934 & -0.406616 & 0.416893\\
-0.0025 & 0.0771983 & -0.336015 & 0.344769\\
-0.002 & 0.0592427	& -0.273882 & 0.273882\\
-0.0014 & 0.0432106 & -0.19544 & 0.20016\\
-0.0013 & 0.0399464 & -0.18019 & 0.184565\\
-0.0012 & 0.0368677 & -0.166894 & 0.170918\\
-0.0011 & 0.0330214 & -0.153018 & 0.156540\\
-0.001 & 0.0290449 & -0.141952 & 0.144893\\
0.00001 & -0.000578125 & 0.00275403 & 0.00281406\\
0.0001 & -0.00369549 & 0.0168763 & 0.0172762\\
0.0002 & -0.00747892 & 0.0329963 & 0.0338333\\
0.0003 & -0.0105089 & 0.0547679 & 0.0557670\\
0.0004 & -0.017467 & 0.0741247 & 0.0761549\\
0.0005 & -0.0206883 & 0.0987991 & 0.100942\\
0.0006 & -0.0296109 & 0.123964 & 0.127451\\
0.0007 & -0.0362697 & 0.159748 & 0.163814\\
0.0008 & -0.0415814 & 0.192351 & 0.196794\\
0.0008 & -0.0459536 & 0.222452 & 0.227149\\
0.001 & -0.0585804 & 0.275473 & 0.281633\\
\hline
\end{tabular}
\label{table:speed1}
\end{center}

We then plotted the graphs of $a_1$ vs $s$ with various lines of best fit to see what relationships are present between these particular parameters. Firstly we plotted the graph of $a_1$ vs $s$ for all but the first 3 values in table \ref{table:speed1}. The first 3 values were discarded as the speed of the wave was such that the wave disappeared quickly from the box. Therefore, it was not possible to get an accurate reading of the speed since there was insufficient quantity of tip plots. We show our the results in figures \ref{fig:speed_fit_lin_quad}, \ref{fig:speed_fit_lin_cub}, \ref{fig:speed_fit_lin_cubodd} and \ref{fig:speed_fit_lin_quad_cub}.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_quadratic.eps}
\caption{Graph of $a_1$ vs $s$ with both a linear and quadratic fit.}
\label{fig:speed_fit_lin_quad}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic.eps}
\caption{Graph of $a_1$ and $s$ with a linear and a cubic fit.}
\label{fig:speed_fit_lin_cub}
\end{minipage}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic_odd.eps}
\caption{Graph of $a_1$ vs $s$ with linear fit and also a cubic fit that is an odd function.}
\label{fig:speed_fit_lin_cubodd}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_quadratic_cubic_odd.eps}
\caption{Graph of $a_1$ and $s$ with all 3 fits (cubic fit is the odd function).}
\label{fig:speed_fit_lin_quad_cub}
\end{minipage}
\end{center}
\end{figure}

Without a doubt, for small \emph{negative} gradients ($a_1$), we get a linear relationship, generated by the line $s=-132.468a_1+0.0121156$.

For positive gradients, it is clear that the relationship is not linear for the range of gradients we have looked at. We fitted a quadratic line to the data to give the equation $s=164802a_1^2+112.671a_1+0.00360838$. However, we believe that a cubic fit is better for our purposes. We generated 2 cubic fits - one with both even and odd terms, and the other with just odd terms. The equations of these cubics are $s=91242700a_1^3+26661.49a_1^2+166.405a_1-0.000487543$ and $s=91242700a_1^3+187.283a_1$. Of course, if $a_1$ is extremly small, we can see that there will be a linear relationship since terms of $O(a_1^2)$ can be neglected.

There is something no quite convincing about the above results. The theory that the speed is proportional to the gradient is an established theory that has been proved. We must therefore conduct further tests in order to establish exactly why the theory does not fit our results.


\subsubsection{Retesting}
\label{sec:retest}

The first task we conducted was a review of the amended code. We checked that the amendments were correctly included in the code and that the code was compiling in the way that it should. Our observations could not see any errors in the code.

However, on looking at the function that generates the initial conditions, we noticed that $a(x)$ was called. Previously, we had just $a$ which was a constant in the original code. Therefore, to elimate this as a possible cause of the discrepancy, we decided to run some tests using $a_0$ in the generation of the initial conditions rather than $a(x)=a_0+a_1x$ using various gradients. Some of our results are depicted in the figures \ref{fig:retest9x}, \ref{fig:retest9y}, \ref{fig:retest12x} and \ref{fig:retest12y}.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx023.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ with original on right and retested version on left ($a_0$ for $a_1$=0.0008 in initial conditions instead of $a(x)$).}
\label{fig:retest9x}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity023.eps}
\end{minipage}
\caption{Graph of $t$ vs $y$ for $a_1$=0.0008 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest9y}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest12.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx017.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ for $a_1$=0.0002 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest12x}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity023.eps}
\end{minipage}
\caption{Graph of $t$ vs $y$ for $a_1$=0.0002 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest12y}
\end{center}
\end{figure}

We can clearly see that the graphs in each figure are exactly the same and therefore we can conclude that it is qualitatively irrelevent whether we use $a_0$ (a constant) or $a(x)$ (a function evaluated at a particular $x$) to generate the initial conditions.

Next we decided to check whether the initial conditions had an effect. There is a further theory to say that if the gradient is inverted, then the initial conditions must also be inverted. So far, the initial conditions have been the same for both positive and negative gradients. We adjusted the code yet again to take this into account and re-ran the experiments.

We took 2 values of gradient for which the speed for the positive gradient is much greater than the speed of the negative gradient, and came up with the following results:

\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
Figure & $a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
Figure \ref{fig:retest13} & 0.001 & -0.0651837 & 0.264594 & 0.272504\\
Figure \ref{fig:retest14} & -0.001 & 0.065026 & -0.274845 & 0.282433\\
\hline
Figure \ref{fig:retest15} & 0.0013 & -0.119214 & 0.430456 & 0.446659\\
Figure \ref{fig:retest16} & -0.0013 & 0.124477 & -0.430456 & 0.448093\\
\hline
\end{tabular}
\label{table:speed2}
\end{center}

We can compare the results in table \ref{table:speed2} to those in the original experiments, which are shown in the following table.

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
0.001 & -0.0637345 & 0.262569 & 0.270194\\
-0.001 & 0.0289989 & -0.141975 & 0.144906\\
\hline
0.0013 & -0.107506 & 0.441938 & 0.454826\\
-0.0013 & 0.0.0403389 & -0.18053 & 0.184982\\
\hline
\end{tabular}
\label{table:speed3}
\end{center}

We can see that the revised figure in table \ref{table:speed3}, clearly fit the theory.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest13.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest13.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=0.001}
\label{fig:retest13}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest14.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest14.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=-0.001}
\label{fig:retest14}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest15.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest15.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=0.0013}
\label{fig:retest15}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest16.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest16.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=-0.0013}
\label{fig:retest16}
\end{center}
\end{figure}

However, it is still rather puzzling as to why the original data did not fit the theory. We therefore decide to try a further test which moved the original initial conditions from its original position by a certain amount of space steps.

Firstly, we took

Finally, we decided to see whether the initial transient from the starting point to when the wave settles down to steady rotations has an effect on the speed of the wave. To do this we initiated a rigidly rotating wave without a gradient, letting the wave settle down and rotate about a fixed point which was as close to the centre of the box as possible. After a few rotations, the wave was stopped and the final conditions file generated by EZSpiral was used as the initial conditions file for the next few simulations. We then started EZSpiral again but this time introducing a gradient and did the usual analysis. Our results are presented in the following table \ref{table:speed4}:

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
-0.0014 & 0.0722856 & -0.289977 & 0.298851\\
-0.0012 & 0.0622736 & -0.239769 & 0.247724\\
-0.001 & 0.0469367 & -0.19443 & 0.200015\\
-0.0008 & 0.0353927 & -0.148323 & 0.152487\\
-0.0004 & 0.0162417 & -0.0690147 & 0.0709001\\
-0.0002 & 0.00673007 & -0.033589 & 0.0342566\\
0.0002	& -0.0076846 & 0.0330261 & 0.0339084\\
0.0004	& -0.0154812 & 0.0675423 & 0.0692938\\
0.0006 & -0.0243027 & 0.10343 & 0.106247\\
0.0008 & -0.0348249 & 0.141664 & 0.145882\\
0.001 & -0.0453209 & 0.183785 & 0.189291\\
0.0012	& -0.0544602 & 0.222769 & 0.229329\\
0.0014 & -0.0690389 & 0.277411 & 0.285873\\
0.0016 & -0.0720951 & 0.314733 & 0.322885\\
0.0018 & -0.0983964 & 0.388473 & 0.400741\\
\hline
\end{tabular}
\label{table:speed4}
\end{center}

Comparing graphically the above data we get the graphs shown in figures \ref{fig:vel_late_grad} and \ref{fig:fit_speed_late_grad}.


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/x_vel_late_grad.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/y_vel_late_grad.eps}
\end{minipage}
\caption{Graphs of $a_1$ vs $\dot{x}$ on the left and the graph of $a_1$ vs $\dot{y}$}
\label{fig:vel_late_grad}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_linear_late_grad.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic_odd_lategrad.eps}
\end{minipage}
\caption{Graphs of $a_1$ vs $speed$ with a linear fit on the left and a cubic fit on the right}
\label{fig:fit_speed_late_grad}
\end{center}
\end{figure}

We can see that these results now fit the theory that the speed is proportional to the gradient a lot better than in the previous cases. We can see that the fits in figure \ref{fig:fit_speed_late_grad} are very much linear fits and hence proving the theory from a numerical point of view.


\subsubsection{Summary for Initial Analysis}
\label{sec:summ}

We have seen that the systems studied in section \ref{sec:numanal} are sensitive to initial conditions. The initial transient before the wave settles down plays a big part in determining the speed of the wave. Therefore, in order to generate accurate results we must get rid of the initial transient by initiating a non-drifting wave that rotates around a point as close to the centre of the box as possible and then introduce a gradient to make the wave drift. This will eliminate any errors produced by the initial transient and therefore give us more accurate numerical results.

\subsection{Equation of motion for the tip of a rigidly rotating wave}

\subsubsection{setting up the equations}

Before moving on to study how drifting MRW's behave, let us consider the motion of the tip of a RW. From Biktashev 1996, we have:

\begin{eqnarray*}
\frac{\partial{\Theta}}{\partial{t}} & = & w_0\\
\frac{\partial{R}}{\partial{t}} & = & c_0e^{i\Theta}
\end{eqnarray*}

Letting $R=x(t)+iy(t)$ and $\Theta=\Theta(t)$ with $x(0)=x_0$, $y(0)=y_0$ and $\Theta(0)=\Theta_0$ gives us:

\begin{eqnarray*}
\frac{\partial{\Theta}}{\partial{t}} & = & w_0\\
\frac{\partial{x}}{\partial{t}} & = & c_0\cos(\Theta)\\
\frac{\partial{y}}{\partial{t}} & = & c_0\sin(\Theta)
\end{eqnarray*}

Solving these and letting $\frac{c_0}{w_0}=R$ yields the following solution:

\begin{eqnarray*}
\Theta & = & w_0t+\Theta_0\\
x & = & x_0+R\sin(w_0t+\Theta_0)\\
y & = & y_0-R\cos(w_0t+\Theta_0)
\end{eqnarray*}

These equations give us the equations of motion for the tip of a rigidly rotating spiral wave. A couple of steps of simple algegra produces:

\begin{eqnarray*}
(x-x_0)^2+(y-y_0)^2 & = & R
\end{eqnarray*}

which fits in with the fact that the tip of a rigidly rotating wave traces out a perfect circle.

Earlier analysis in section \ref{sec:numanal} used $x(t)=x_0+c_xt$ and $y(t)=y_0+c_yt$ to produce a straight to determine the speed of the drifting wave. In fact, we can say that these linear equations are the actual equations of motion for the point of rotation of the drifting wave. Theresfore, we propose that the equations of motion for a rigidly rotating spiral wave that drifts are:

\begin{eqnarray*}
x & = & x_0+c_xt+R\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt-R\cos(w_0t+\Theta_0)
\end{eqnarray*}

\noindent For our purposes we now suppose that:

\begin{eqnarray*}
x & = & x_0+c_xt+R_x\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt-R_y\cos(w_0t+\Theta_0)
\end{eqnarray*}
\\
and we should find that $R_x=R_y=R$.

\subsubsection{Numerical Testing of these equations}

Throughout our testing, we used Gnuplot to fit the equations to the data. However, Gnuplot is very sensitive to initial conditions and therefore we need to make a good initial estimate of what the parameters in the equations are going to be. These initial estimates, together with the results, are shown in the following subsections.

\subsubsection{y component}

Let us firstly consider fitting $y(t)$ to the $y$ component of the tip data for the gradient $a_1$=-0.0002. In order to generate a fairly accurate fitted function, we need to specify some initial hand calculated values for each of the 5 parameters. These were calculated to be:

\begin{eqnarray*}
x_0 & = & 29.9976 \\
c_x & = & -0.0336148 \\
R_x & = & 3.5 \\
\omega_x & = & 0.636809 \\
\phi_x & = & -1.37304 
\end{eqnarray*}

Firstly, it is noted that our value of $a_1$ is small and therefore the speed of the drift if also small and fits with the theory that it is linearly dependent on the gradient. Next, we conducted several fitting procedures. The first procedure used the data from just a few rotations of the wave. This was in order to see if the fitting procedure was working. The next procedure was for a few more rotations whilst the final procedure fitted the function to many rotations. Our results are shown below.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity1.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity10.eps}
\end{minipage}
\caption{Here we fit the function over just a handful of rotations and get the function $y(t)=29.9369-0.032849t+3.5244\sin(0.636348t+0.915195)$, with $y(t)$ coinciding with the orginal trajectory on the left and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity1}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity2.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity3.eps}
\end{minipage}
\caption{The same function as in figure \ref{fig:fity1} is plotted here but the plotting on the above graphs is now over a wider range of time steps. as with figure \ref{fig:fity1}, the graph on the left has both the orginal trajectory and $y(t)$ coinciding and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity2}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity4.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity5.eps}
\end{minipage}
\caption{We now fit the function over more rotations (double the amount of the first fit) and get $y(t)=29.9519-0.0332139t+3.52898\sin(0.635567t+0.947123)$. We can see that the fitted function, $y(t)$, coincides with the orginal trajectory on the left and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity3}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity6.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity7.eps}
\end{minipage}
\caption{We now fit the function over 4 times as many rotations than in the second fit shown in figure \ref{fig:fity3} above and get $y(t)=29.9864-0.0335229t+3.47646\sin(0.631333t+1.45241)$. We plot both the orginal trajectory and the fitted function, $y(t)$ over the same range and get the above graphs.}
\label{fig:fity4}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity8.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fity9.eps}
\end{minipage}
\caption{Here we keep the function found in figure \ref{fig:fity4} but plot both the original trajectory and $y(t)$ over shorter domains.}
\label{fig:fity5}
\end{center}
\end{figure}

It is clear from figures \ref{fig:fity4} and \ref{fig:fity5} that for some reason Gnuplot is not giving us accurate plots for larger domains. This could be down to the fact that because the domain is large then the plot is less accurate. Over shorter domains we get that the fitted function is almost a perfect fit. Hence to combat this, we need to adjust the accuracy in Gnuplot.

\subsubsection{x component}

Let us now do the same for the x component. The initial values are:


\begin{eqnarray*}
x_0 & = & 30.0668 \\
c_x & = & 0.00675554 \\
R_x & = & 3.51 \\
\omega_x & = & 0.636809 \\
\phi_x & = & 1.00 
\end{eqnarray*}

The results are now as follows.


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx1.eps}
\end{minipage}
\caption{Here we fit the function over just a handful of rotations as with figure \ref{fig:fity1} and get the function $x(t)=30.1547+0.00699495t+3.52158\sin(0.63638t-2.22774)$.}
\label{fig:fitx1}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx2.eps}
\end{minipage}
\caption{The same function as in figure \ref{fig:fity1} is plotted here but the plotting on the above graphs is now over a wider range of time steps. as with figure \ref{fig:fitx1}.}
\label{fig:fitx2}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx3.eps}
\end{minipage}
\caption{We now fit the function over more rotations (double the amount of the first fit) and get $x(t)=30.1791+0.00633029t+3.52665\sin(0.635589t-2.19654)$.}
\label{fig:fitx3}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx4.eps}
\end{minipage}
\caption{We now fit the function over 4 times as many rotations than in the second fit shown in figure \ref{fig:fitx3} above and get $x(t)=30.1328+0.00642943t+3.46909\sin(0.631311t-1.68495)$.}
\label{fig:fitx4}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx5.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitx6.eps}
\end{minipage}
\caption{Here we keep the function found in figure \ref{fig:fitx4} but plot both the original trajectory and $x(t)$ over shorter domains.}
\label{fig:fitx5}
\end{center}
\end{figure}

\subsubsection{Comparing results}

Let us now compare some of the results. We should find that $R_x$ and $R_y$ are the same as should be $\omega_x$ and $\omega_y$ together with $\phi_x$ and $\phi_y$. Consider the following table.

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Figure and component & $x_0$/$y_0$ & $c_x$/$c_y$ & $R_x$/$R_y$ & $\omega_x$/$\omega_y$ & $\phi_x$/$\phi_y$\\
\hline
Figure \ref{fig:fitx1} and x comp. & 29.9369 & -0.032849 & 3.5244 & 0.636348 & 0.915195\\
Figure \ref{fig:fity1} and y comp. & 30.1547 & 0.00699495 & 3.52158 & 0.63638 & -2.22774\\
\hline
Figure \ref{fig:fitx3} and x comp. & 29.9519 & -0.0332139 & 3.52898 & 0.635567 & 0.947123\\
Figure \ref{fig:fity3} and y comp. & 30.1791 & 0.00633029 & 3.52665 & 0.635589 & -2.19654\\
\hline
Figure \ref{fig:fitx4} and x comp. & 29.9864 & -0.0335229 & 3.47646 & 0.631333 & 1.45241\\
Figure \ref{fig:fity4} and y comp. & 30.1328 & 0.00642943 & 3.46909 & 0.631311 & -1.68495\\
\hline
\end{tabular}
\label{table:speed}
\end{center}
\end{footnotesize}

Clearly, $R_x$ and $R_y$ are almost the same as are $\omega_x$ and $\omega_y$. We can see that $\phi_x$ and $\phi_y$ are not the same. However, the difference between them is $\pi$ in each case. Therefore, taking the angle of the $x$-component to be $\theta$, this gives the $y$-component to be $\theta-\pi$. Hence,

\begin{eqnarray*}
\cos(\theta-\pi) & = & \cos(\theta)\cos(\pi)+\sin(\theta)\sin(\pi)\\
& = & -\cos(\theta)
\end{eqnarray*}
\\
implying that the sign in front of cos in the equation of motion for $y$ is changed giving the folowing revised equations of motion:

\begin{eqnarray*}
x & = & x_0+c_xt+R_x\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt+R_y\cos(w_0t+\Theta_0)
\end{eqnarray*}



\subsection{Meandering Waves}

We have now established that EZSpiral is working correctly for rigidly rotating waves and how we should conduct future experiments. We now move on to drifting MRW's and see what results we get. Note that this area has not been touched before and the results produced are original.


subsection{Non-Drifting Meandering Waves}
We know that MRW's are quasiperiodic. Let us assume that the equations of motion are:

\begin{eqnarray*}
x(t) & = & x_0+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}

We showed in the exercise for Rigidly Rotating waves that $R_x$ and $R_y$ are in fact the same (say $R$) as are $\omega_{1x}$ and $\omega_{1y}$ ($\omega_1$). Let us assume that $r_x$ and $r_y$ ($r$ say) are the same and also $\omega_{2x}$ and $\omega_{2y}$ are also the same ($\omega_2$). Note that $R$ and $\omega_1$ are the primary radius and primary frequency respectively, and $r$ and $\omega_2$ are the secondary radius and frequency (i.e the radius and frequency in the rotating frame of reference).

Looking at the tip file and also at the graph of the trajectory of the wave (see figure \ref{fig:mrw41}) we get the following initial estimates of the various parameters:

\begin{eqnarray*}
x_0 & = & 28.73429 \\
y_0 & = & 28.50880 \\
R & = & 3.25 \\
\omega_1 & = & 0.162496 \\
\phi_1 & = & 1.00\\
r & = & 0.9\\
\omega_2 & = & 1.65\\
\phi_2 & = & 0.8  
\end{eqnarray*}


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/mrw041.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/mrw041_part.eps}
\end{minipage}
\caption{Graphs of the trajectories for a non-drifting meandering wave with the full trajectory on the left and a part trajectory (1 full rotation) on the right.}
\label{fig:mrw41}
\end{center}
\end{figure}

Preliminary results using these initial estimates by Gnuplot are shown in figure \ref{fig:mrw41fit}.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwy41.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwx41.eps}
\end{minipage}
\caption{Fit by Gnuplot for both $x(t)$ and $y(t)$.}
\label{fig:mrw41fit}
\end{center}
\end{figure}

 It is clear that this function fits the data and the equations are given by:

\begin{eqnarray*}
x(t) & = & 30.1294+2.88181\cos(0.167468t-0.683533)\\
&& +0.798711\cos(1.63341t+0.595935)\\
y(t) & = & 30.2545+2.93476\sin(0.16552t-0.597004)\\
&& -0.792184\sin(1.63692t+0.437389)
\end{eqnarray*}

These functions are fitted just for 1 rotation. Let us consider more than one rotation as shown in figure \ref{fig:mrw41fitmore}.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwx41more.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwy41more.eps}
\end{minipage}
\caption{Fit by Gnuplot for both $x(t)$ on the left and $y(t)$ on the right for more than 1 rotation (just over 3).}
\label{fig:mrw41fitmore}
\end{center}
\end{figure}

It is clear that this function fits the data and the equations are given by:

\begin{eqnarray*}
x(t) & = & 30.1212+2.89537\cos(0.167333t-0.674339)\\
&& +0.799068\cos(1.63446t+0.544719)\\
y(t) & = & 30.356+2.9127\sin(0.167285t-0.675932)\\
&& -0.794017\sin(1.63477t+0.531315)
\end{eqnarray*}

This is a more accurate fit. We can see that the parameters $R_x$, $r_x$, $\omega_{1x}$, $\omega_{2x}$, $\phi_{1x}$ and $\phi_{2x}$ to 3 signigificant figures can be said to be the same as their $y$ counterparts with the difference being less than 1\%. We conclude that for a meandering spiral wave with a stationary point of rotation we can generate the equation of the tip of the wave with the above equations.

\subsubsection{Drifting Meandering Wave}

We saw above that a meandering wave whose point of rotation is fixed can be approximated using the following equations:

\begin{eqnarray*}
x(t) & = & x_0+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}

We propose that the equations of drifting meandering waves are given by:

\begin{eqnarray*}
x(t) & = & x_0+c_xt+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+c_yt+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}

The only difference being the velocity components for $x$ and $y$. To put this proposition to the test, let us take the data for when the gradient is $a_1$=0.0004. We will use the following initial estimates of the parameters.

\begin{eqnarray*}
x_0 & = & 28.73429 \\
y_0 & = & 28.50880 \\
c_x & = & -0.00763589\\
c_y & = & -0.0104151\\
R & = & 3.25 \\
\omega_1 & = & 0.162496 \\
\phi_1 & = & 1.00\\
r & = & 0.9\\
\omega_2 & = & 1.65\\
\phi_2 & = & 0.8  
\end{eqnarray*}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/mrw002.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/mrw002_part.eps}
\end{minipage}
\caption{Graphs of the trajectories for a drifting meandering wave with the full trajectory on the left and a part trajectory (2 full rotation) on the right.}
\label{fig:mrw002}
\end{center}
\end{figure}

We can see from figure \ref{fig:mrw002} that the wave is moving to the bottom left and actually moves rather slowly. Let us see how Gnuplot fits these functions.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwx002.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/inhom/fitmrwy002.eps}
\end{minipage}
\caption{The above graphs show how the functions were fitted to the data with $x(t)$ on the left and $y(t)$ on the right.}
\label{fig:mrw002fit}
\end{center}
\end{figure}

From the graphs in figure \ref{fig:mrw002fit}, we can see that Gnuplot has fitted the functions quite well. The functions take the form:

\begin{eqnarray*}
x(t) & = & 30.4127-0.00805152t+2.91423\cos(0.166231t-0.676989)\\
&&+0.795599\cos(1.63444t+0.571694)\\
y(t) & = & 29.9896-0.0107487t+2.92391\sin(0.166176t-0.666409)\\
&& +0.793362\sin(1.63461t-2.59023)
\end{eqnarray*}

\subsection{Conclusion}

We can conclude from the results present in this section, that the general form of the equations of motion for the tip of a meandering wave that drifts is:

\begin{eqnarray*}
x(t) & = & x_0+c_xt+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+c_yt+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}

\noindent This was shown to be true numerically and therefore we need to show it is true analytically.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Resonance - Numerical Work - pictures}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/traj.eps}
\end{minipage}
\caption{Meandering Spiral Wave drifting due to inhomogeneities, passing through a point of resonance.}
\label{fig:traj}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/quotient.eps}
\end{minipage}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cx_cy.eps}
\end{minipage}
\caption{The plot of the quotient system on the left and $c_x$ against $c_y$ on the right.}
\label{fig:quot}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cx_vs_om.eps}
\end{minipage}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cy_vs_om.eps}
\end{minipage}
\caption{$c_x$ against $\omega$ on the left and $c_y$ against $\omega$ on the right.}
\label{fig:quot1}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/speed.eps}
\end{minipage}
\caption{$\frac{dx}{dt}$ versus $\frac{dy}{dt}$.}
\label{fig:speed}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/poincare_0.008.eps}
\end{minipage}
\caption{The Poincare Cross Section. Time is plotted on the horizontal axis and $y$ on the vertical.}
\label{fig:pcs}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Behaviour around a point of resonance}

\subsection{Introduction}
\label{ch:intro2}

In this analysis we look at how the meandering spiral wave behaves near points of resonances when we induce the wave to drift by applying a gradient. Meandering spiral waves are quasiperiodic solutions to the governing equations and therefore we must have that the two frequencies are not rationally related, i.e.
\[\frac{\omega_1}{\omega_2} \neq \frac{p}{q} \hfill \mbox{ s.t. } p,q \in \mathbb{Z}\]
We find however that we come across frequencies that are almost rationally related but not quite, and the parameters for which this occurs give us the point of resonance.

In this analysis, we will take the parameters $a_0=0.01875$, $b=0.01$ and $\epsilon =0.01$, which almost gives us a 4:1 resonance, i.e. the secondary frequency is 4 times that of the primary frequency (the actual ratio is approximately 4.027:1).

\subsubsection{Initial Analysis}

As usual, we have kept the parameters $a_0$ and $\epsilon$ fixed and vary the gradient, $a_1$. We also use the technique developed previous reports whereby we initate the wave with the centre of rotation as close to the centre of the domain as possible. We display the initial trajectories in Figs. \ref{fig:mrwres001} to \ref{fig:mrwres013}, with the trajectory in Fig. \ref{fig:mrwres001} being the meandering spiral wave with no gradient applied and therefore it does not drift. Also, in Fig. \ref{fig:mrwres001} we have include just 2 full rotations and it can been seen on closer inspection that there are almost exactly 4 inward facing ``petals" corresponding to the 4:1 resonance.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres001.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres002.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres003.eps}
\end{minipage}
\caption{(left) $a_1=0$; (center) $a_1=0.0002$; (right) $a_1=0.0004$.}
\label{fig:mrwres001}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres004.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres005.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres006.eps}
\end{minipage}
\caption{(left) $a_1=0.0006$; (center) $a_1=0.0008$; (right) $a_1=0.001$.}
\label{fig:mrwres004}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres007.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres008.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres009.eps}
\end{minipage}
\caption{(left) $a_1=0.0012$; (center) $a_1=0.0014$; (right) $a_1=-0.0002$.}
\label{fig:mrwres007}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres010.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres011.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres012.eps}
\end{minipage}
\caption{(left) $a_1=-0.0004$; (center) $a_1=-0.0006$; (right) $a_1=0.0008$.}
\label{fig:mrwres010}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres013.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres014.eps}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres015.eps}
\end{minipage}
\caption{(left) $a_1=-0.001$; (center) $a_1=-0.0012$; (right) $a_1=-0.0014$.}
\label{fig:mrwres013}
\end{center}
\end{figure}

Initial observations show that near a point of resonance, the spiral wave does not behave like what we have previously observed in other numerical experiments. We can see from Fig. \ref{fig:mrwres001}(center) that the wave almost looks as though it behaves like a Rigidly Rotating spiral wave for the first part of the trajectory but in fact on closer inspection we can see that the trajectory slightly oscilates from side to side as it progresses, which is due to the presence of the secondary frequency.

Then, as the wave reaches a certain point, it's trajectory changes. We have split up this trajectory to demonstrate this behaviour in more detail and this is shown in Figs. \ref{fig:reson2} to \ref{fig:reson5}.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/reson2.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/reson3.eps}
\end{minipage}
\caption{Trajectory for $a_1=0.0002$: first part (left); final part (right).}
\label{fig:reson2}
\end{center}
\end{figure}


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/reson4.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/reson5.eps}
\end{minipage}
\caption{A few rotations of the wave as we just get into the last part of the trajectory for $a_1=0.0002$ (left); a few more rotations (right).}
\label{fig:reson5}
\end{center}
\end{figure}

As we can see, once the wave reaches this particular point, the meandering motion of the wave is greatly exagerated and also the wave changes direction. As we increase the gradient, $a_1$, we can see that this phenominem changes - the direction of motion changes, the severity of the change of motion also changes.

Once we reach a certain value of the gradient, it can be seen that we no longer get this phenominem but the spiral wave drifts out of the domain. Also, as the gradient increases, the direction of travel also increases. Whether this change is proportional to the gradient has yet to be investigated. Also, for $a_1=\pm 0.0014$, we observe that the trajectory generated is very strange. This appears to be due to the fact that in this particular instance the gradient is too large. Again, further investigation is needed.

Furthermore, for $a_1=\pm 0.0004$, the trajectory of the wave looks as though it bends to the right for the positive value and to the left for the negative value. Further investigation is also needed in this instance.

Initially, we thought that the boudaries may have an affect and cause the phenominem described above. Therefore, we ran the experiment in a larger domain for $a_1=0.0002$ ($L_x$ was now to be increased from 60 to 120 and the number of points, $N_x$, increased from 181 to 361 - therefore the space step was kept constant). We can see from Fig. \ref{fig:mrwres016}, that the same phenominem occurs. The trajectory begins as in the smaller domain, looking as though it is moving like a Rigidly Rotating wave. Then once it gets to a certain point, it changes direction and the trajectory gets wider. This is as per the smaller domain, so therefore we can say that the phenominem may not depend on the domain size and nor does the boundary have an influence.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.75\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwres016.eps}
\caption{Trajectory of the spiral wave for $a_1$=0.0002 in a larger domain.}
\label{fig:mrwres016}
\end{minipage}
\end{center}
\end{figure}

Finally, we show the tajectories for both time against $x$ and also time against $y$ in Figs. \ref{fig:mrwresx002} and \ref{fig:mrwresy002}. Clearly, when the trajectory reaches a particular point, it changes direction and shape. It looks as though the primary radius (i.e. the radius of the circle in the absence of the secondary frequency) has actually increased. This needs to be looked at in more detail together with whether the speed of the wave is proportional to the gradient as per previous analysis.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwresx002.eps}
\caption{Time against $x$\newline for $a_1=0.0002$.}
\label{fig:mrwresx002}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/initial_numerics/resonance1/mrwresy002.eps}
\caption{Time against $y$\newline for $a_1=0.0002$.}
\label{fig:mrwresy002}
\end{minipage}
\end{center}
\end{figure}

\subsubsection{Brief Summary}

To conclude this brief report we can summarise as follows:

$\bullet$ For small gradients there are points at which the trajectory of the wave changes.\\
$\bullet$ For different values of the gradient, we get the wave travelling in different directions.\\
$\bullet$ For large gradient, we do not observe the phenominem seen for small gradients.\\
$\bullet$ Initial observations suggest that the boundaries are not responsible for this phenominem.

Further investigation is needed on the following.

$\bullet$ Is the direction of the wave for various gradients proportional to the gradient?\\
$\bullet$ At what point does the observed phenominem cease?\\
$\bullet$ Various other parameter ($a_0$ and $b$) needed to investigated to see if there are so called "tongues" in which this phenominem occurs.\\
$\bullet$ What is the maximum gradient that can be applied in this instance to get a meaningful result and is this dependent on the other parameters?\\
$\bullet$ Why does the trajectory curve to the right (left) for $a_1$=0.0004(=-0.0004)?\\
$\bullet$ Is the speed of the wave proportional to the gradient?\\
$\bullet$ How does the primary radius change and to what extent does it change for various gradients?

==> chapter2/defs.tex <==
\newtheorem{thm}{Theorem}[section]

\theoremstyle{definition}	

\newtheorem{defn}[thm]{Definition}

\newcommand{\ez}{EZ-Freeze }

%%%%%%%%%%%%%%%%% Group Actions etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dd}{\textrm{d}}
\newcommand{\dT}{\textrm{T}(g)}
\newcommand{\ddT}{\textrm{T}(dg)}
\newcommand{\dTddT}{\textrm{T}(g+dg)}
\newcommand{\dTi}{\textrm{T}(g^{-1})}
\newcommand{\ddTi}{\textrm{T}(dg^{-1})}
\newcommand{\ddTcom}{\textrm{T}(\{\textbf{c}dt,\omega dt\})}

%%%%%%%%%%%%%%%%% Bold letters and Symbols %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Greek

\newcommand{\balp}{\boldsymbol{\alpha}}
\newcommand{\bbet}{\boldsymbol{\beta}}
\newcommand{\bet}{\boldsymbol{\eta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

%Latin

\newcommand{\bA}{\textbf{A}}
\newcommand{\bD}{\textbf{B}}
\newcommand{\bc}{\textbf{c}}
\newcommand{\bC}{\textbf{C}}
\newcommand{\be}{\textbf{e}}
\newcommand{\bof}{\textbf{f}}
\newcommand{\boof}{\textbf{f}}
\newcommand{\booF}{\textbf{F}}
\newcommand{\boF}{\textbf{F}(\textbf{V})}
\newcommand{\boFU}{\textbf{F}(\textbf{U})}
\newcommand{\boFt}{\textbf{F}(\textbf{t})}
\newcommand{\bFg}{\textbf{F}_{\mathcal{G}}(\bV)}
\newcommand{\bFm}{\textbf{F}_{\mathcal{M}}(\bV)}
\newcommand{\bg}{\textbf{g}}
\newcommand{\bG}{\textbf{G}}
\newcommand{\bGt}{\textbf{G}(\textbf{t})}
\newcommand{\bh}{\textbf{h}}
\newcommand{\bH}{\textbf{H}}
\newcommand{\bHg}{\til{\bH}_{\mathcal{G}}(\bV,t)}
\newcommand{\bHm}{\til{\bH}_{\mathcal{M}}(\bV,t)}
\newcommand{\bI}{\textbf{I}}
\newcommand{\bk}{\textbf{k}}
\newcommand{\bM}{\textbf{M}}
\newcommand{\bP}{\textbf{P}}
\newcommand{\bp}{\textbf{p}}
\newcommand{\bq}{\textbf{q}}
\newcommand{\bQ}{\textbf{Q}}
\newcommand{\br}{\textbf{r}}
\newcommand{\bR}{\textbf{R}}
\newcommand{\bS}{\textbf{S}}
\newcommand{\bu}{\textbf{u}}
\newcommand{\bU}{\textbf{U}}
\newcommand{\bv}{\textbf{v}}
\newcommand{\bV}{\textbf{V}}
\newcommand{\bw}{\textbf{w}}
\newcommand{\bW}{\textbf{W}}

%%%%%%%%%%%%%%%%% letters with hats and tildes %%%%%%%%%%%%%%%%%

\newcommand{\til}{\tilde}
\newcommand{\bDh}{\hat{\textbf{D}}}
\newcommand{\Bh}{\hat{\partial}}
\newcommand{\hh}{\hat{\textbf{h}}}
\newcommand{\bHt}{\tilde{\textbf{H}}(\textbf{V},t)}
\newcommand{\tH}{\tilde{\textbf{H}}}
\newcommand{\bht}{\tilde{\textbf{h}}}
\newcommand{\btr}{\tilde{\textbf{r}}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tr}{\tilde{r}}
\newcommand{\tbr}{\tilde{\textbf{r}}}
\newcommand{\ttim}{\tilde{t}}
\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tth}{\tilde{\theta}}

%%%%%%%%%%%%%%%%% Derivatives %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\deriv}[2]{\frac{\dd #1}{\dd #2}}

%ODE's

\newcommand{\odcxot}{\frac{\dd{\bc_{x0}}}{\dd{t}}}
\newcommand{\odcyot}{\frac{\dd{\bc_{y0}}}{\dd{t}}}
\newcommand{\odcot}{\frac{\dd{\bc_0}}{\dd{t}}}
\newcommand{\odomt}{\frac{\dd{\omega}}{\dd{t}}}
\newcommand{\odRt}{\frac{\dd{R}}{\dd{t}}}
\newcommand{\odbRt}{\frac{\dd{\bR}}{\dd{t}}}
\newcommand{\odTt}{\frac{\dd{\dT}}{\dd{t}}}
\newcommand{\odTht}{\frac{\dd{\Theta}}{\dd{t}}}
\newcommand{\odThot}{\frac{\dd{\Theta_0}}{\dd{t}}}
\newcommand{\odThonet}{\frac{\dd{\Theta_1}}{\dd{t}}}
\newcommand{\odbut}{\frac{\dd{\bu}}{\dd{t}}}
\newcommand{\odbUt}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odut}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odbvt}{\frac{\dd{\bv}}{\dd{t}}}
\newcommand{\odbVt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbVot}{\frac{\dd{\bV_0}}{\dd{t}}}
\newcommand{\odbVpt}{\frac{\dd{\bV_1}}{\dd{t}}}
\newcommand{\odvt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbvpit}{\frac{\dd{\bv}_{pi}}{\dd{t}}}
\newcommand{\odbVpit}{\frac{\dd{\bV}_{1pi}}{\dd{t}}}
\newcommand{\odbwt}{\frac{\dd{\bw}}{\dd{t}}}
\newcommand{\odbWt}{\frac{\dd{\bW}}{\dd{t}}}
\newcommand{\odXt}{\frac{\dd{X}}{\dd{t}}}
\newcommand{\odYt}{\frac{\dd{Y}}{\dd{t}}}

%PDE's - wrt x

\newcommand{\pdbvx}{\frac{\partial{\textbf{v}}}{\partial{x}}}
\newcommand{\pdbux}{\frac{\partial{\textbf{u}}}{\partial{x}}}
\newcommand{\pdux}{\frac{\partial{u}}{\partial{x}}}
\newcommand{\pdvx}{\frac{\partial{v}}{\partial{x}}}
\newcommand{\pdvxk}{\frac{\partial{v^{(i)}_k}}{\partial{x}}}
\newcommand{\pduox}{\frac{\partial{\textbf{u}_0}}{\partial{x}}}
\newcommand{\pdvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbtvox}{\frac{\partial{\til{\textbf{v}}_0}}{\partial{x}}}
\newcommand{\pdvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{x}}}}
\newcommand{\pdbvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\til{x}}}}
\newcommand{\pdvoxx}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}^2}}
\newcommand{\pdtrtx}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{x}}}}
\newcommand{\pdtthtx}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{x}}}}
\newcommand{\pdtxx}{\frac{\partial{\tilde{x}}}{\partial{x}}}
\newcommand{\pdtyx}{\frac{\partial{\tilde{y}}}{\partial{x}}}
\newcommand{\pdax}{\frac{\partial{\alpha}}{\partial{x}}}

%PDE's - wrt y

\newcommand{\pdbvy}{\frac{\partial{\textbf{v}}}{\partial{y}}}
\newcommand{\pduoy}{\frac{\partial{\textbf{u}_0}}{\partial{y}}}
\newcommand{\pdvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\til{y}}}}
\newcommand{\pdvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{y}}}}
\newcommand{\pdvoyy}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}^2}}
\newcommand{\pdtrty}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{y}}}}
\newcommand{\pdtthty}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{y}}}}
\newcommand{\pdtxy}{\frac{\partial{\tilde{x}}}{\partial{y}}}
\newcommand{\pdtyy}{\frac{\partial{\tilde{y}}}{\partial{y}}}

%PDE's - wrt theta

\newcommand{\pdbvth}{\frac{\partial{\textbf{v}}}{\partial{\theta}}}
\newcommand{\pdvoth}{\frac{\partial{\textbf{v}_0}}{\partial{\theta}}}
\newcommand{\pdvth}{\frac{\partial{\textbf{v}_1}}{\partial{\theta}}}
\newcommand{\pdvotth}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{\theta}}}}
\newcommand{\pdvothth}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}^2}}

%PDE's - wrt t

\newcommand{\pdvvtt}{\frac{\partial{\textbf{v}}_1}{\partial{\tilde{t}}}}
\newcommand{\pduot}{\frac{\partial{\textbf{u}_0}}{\partial{t}}}
\newcommand{\pdbut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvot}{\frac{\partial{\textbf{v}_0}}{\partial{t}}}
\newcommand{\pdvott}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{t}}}}
\newcommand{\pdtthtt}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{t}}}}
\newcommand{\pdut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvt}{\frac{\partial{\textbf{v}}}{\partial{t}}}

%PDE's - wrt u/v/U/V

\newcommand{\pdfa}{\frac{\partial{\textbf{f}}}{\partial{\alpha}}}
\newcommand{\pdfu}{\frac{\partial{\textbf{f}}}{\partial{\bu}}}
\newcommand{\pdfvov}{\frac{\partial{\textbf{f}(\textbf{v}_0)}}{\partial{\textbf{v}}}}
\newcommand{\pdgu}{\frac{\partial{\textbf{g}}}{\partial{\bV}}}

%PDE's mixed

\newcommand{\pdvoxy}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{y}}}
\newcommand{\pdvoxth}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{\theta}}}
\newcommand{\pdvoyx}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{x}}}
\newcommand{\pdvoyth}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{\theta}}}
\newcommand{\pdvothx}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{x}}}
\newcommand{\pdvothy}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{y}}}


==> chapter2/spiral_dynamics/initial_numerics/inhom_numerics.tex <==
\section{Numerical Analysis of Spiral Waves that Drift due to Inhomogeneities}

\section{Introduction}
\label{ch:intro}

In this chapter we study the drift of a spiral wave due to in homogeneities. We will firstly present the numerical work that we have carried out together with some preliminary results and conclusions, before providing an analytical approach to this particular area.\\
\\
This project is primarily concerned with meandering spiral waves that drift due to inhomogeneities, but in order to get a feel of what drift due to inhomogeneities entails, we will look at rigid rotation before meander. EZSpiral is yet again used to help us in the numerical analysis of this particular area. When a wave drifts due to inhomogeneities (from now on I will simply say "drift" to mean "drift due to inhomogeneities"), it's parameters are dependant on the spatial coordinates. It's point of rotation is no longer stationary but drifts along a straight line. Therefore we have that $a=a(x,y)$.\\
\\
We then adjusted the code to EZSpiral to take this dependency into account. Initally, we take $a=a_0+a_1x$ so that $a$ is linearly dependant on $x$ only. This now means that we have 4 parameters - $\epsilon,\ a_0,\ a_1,\ b$. Throughout this analysis we take $\epsilon=0.01$, as per previous work.\\


\section{Numerical Analysis}
\label{sec:numanal}

As mentioned in the introduction to this chapter, we are firstly going to look at rigid rotation (RW). Recall, that RW's are periodic solutions to the PDE system being studied. Their tips trace out a perfect circle. When viewed in a rotating frame of reference that rotates with a frequency equal to the frequency of the RW's, they appear to be stationary (a dot is abserved). This type of spiral is the simplest type of spiral to study from a Mathematical point of view and we will consider this firstly.\\

\subsection{Initial Analysis}

Using the parametric portrait obtained in the previous chapter, we chose $a_0,\ a_1,\ \&\ b$, such that we get a RW with a medium core radius. We therefore chose the following values:\\

\begin{eqnarray*}
a_0 & = & 0.7\\
a_1 & = & 0\\
b & = & 0.15\\
\epsilon & = & 0.01
\end{eqnarray*}
\\
Other numerical and physical parameters were chosen as follows:\\

\begin{eqnarray*}
N_x & = & 181\\
L_x & = & 60\\
\mbox{Steps per plot} & = & 16\\
ts & = & 0.8
\end{eqnarray*}
\\
where $ts$ is timestep as a fraction of the diffusion stability limit. This means that our space step and time step were $h_x=\frac{1}{3}$ and $h_t=\frac{1}{30}$ respectively. These steps were kept constant throughout our analysis.\\
\\
First of all we need to show that our amended EZSpiral ran correctly. We therefore ran the program for various values of $a_0$ with $a_1=0$. These runs were then compared to the original data using the original program. The results showed that the amended program gave exactly the same results as the original program. A couple of tests are shown below. Therefore, early indications show that the program is working correctly.\\
\\
There is an established theory which states that for small gradients the speed of the wave is proportional to the gradient. Therefore, in order to test whether EZSpiral is certainly working correctly, we are to prove, numerically, this theory.\\
\\
Firstly, we ran the program for a range of gradients, $a_1$. As usual, a \emph{tip.dat} file is produced from which we can extract a variety of information. We then calculated the "speed" of the wave using the tip file by plotting $t$ vs $x$ and $t$ vs $y$ using Gnuplot and made Gnuplot include a line of best fit. Several examples of these are included in figures \ref{fig:fitxy020} and \ref{fig:fitxy016}. The gradient of this line would then give me $\frac{dx}{dt}$ and $\frac{dy}{dt}$. Using $s=\sqrt{\dot{x}^2+\dot{y}^2}$, where $s$ is the speed of the wave and the "dots" represent the usual differentiation with respect to t, we then plotted $s$ vs gradient ($a_1$) and then observed what relationship(s), if any, are present.\\

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx020.eps}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity020.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and $t$ vs $y$ on the right for $a_1=0.0005$}
\label{fig:fitxy020}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx016.eps}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity016.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and $t$ vs $y$ on the right for $a_1=0.0009$}
\label{fig:fitxy016}
\end{center}
\end{figure}

\noindent From the Gnuplot output and also using Maple to quickly calculate $s$, we get the following table of results:\\

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & s\\
\hline
-0.0038 & 0.111062 & -0.47453 & 0.487253\\
-0.00375 & 0.118094 & -0.513751 & 0.527149\\
-0.0035 & 0.150046	& -0.463961 & 0.487620\\
-0.003 & 0.0919934 & -0.406616 & 0.416893\\
-0.0025 & 0.0771983 & -0.336015 & 0.344769\\
-0.002 & 0.0592427	& -0.273882 & 0.273882\\
-0.0014 & 0.0432106 & -0.19544 & 0.20016\\
-0.0013 & 0.0399464 & -0.18019 & 0.184565\\
-0.0012 & 0.0368677 & -0.166894 & 0.170918\\
-0.0011 & 0.0330214 & -0.153018 & 0.156540\\
-0.001 & 0.0290449 & -0.141952 & 0.144893\\
0.00001 & -0.000578125 & 0.00275403 & 0.00281406\\
0.0001 & -0.00369549 & 0.0168763 & 0.0172762\\
0.0002 & -0.00747892 & 0.0329963 & 0.0338333\\
0.0003 & -0.0105089 & 0.0547679 & 0.0557670\\
0.0004 & -0.017467 & 0.0741247 & 0.0761549\\
0.0005 & -0.0206883 & 0.0987991 & 0.100942\\
0.0006 & -0.0296109 & 0.123964 & 0.127451\\
0.0007 & -0.0362697 & 0.159748 & 0.163814\\
0.0008 & -0.0415814 & 0.192351 & 0.196794\\
0.0008 & -0.0459536 & 0.222452 & 0.227149\\
0.001 & -0.0585804 & 0.275473 & 0.281633\\
\hline
\end{tabular}
\label{table:speed1}
\end{center}

\noindent We then plotted the graphs of $a_1$ vs $s$ with various lines of best fit to see what relationships are present between these particular parameters. Firstly we plotted the graph of $a_1$ vs $s$ for all but the first 3 values in table \ref{table:speed1}. The first 3 values were discarded as the speed of the wave was such that the wave disappeared quickly from the box. Therefore, it was not possible to get an accurate reading of the speed since there was insufficient quantity of tip plots. We show our the results in figures \ref{fig:speed_fit_lin_quad}, \ref{fig:speed_fit_lin_cub}, \ref{fig:speed_fit_lin_cubodd} and \ref{fig:speed_fit_lin_quad_cub}.\\

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_quadratic.eps}
\caption{Graph of $a_1$ vs $s$ with both a linear and quadratic fit.}
\label{fig:speed_fit_lin_quad}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic.eps}
\caption{Graph of $a_1$ and $s$ with a linear and a cubic fit.}
\label{fig:speed_fit_lin_cub}
\end{minipage}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic_odd.eps}
\caption{Graph of $a_1$ vs $s$ with linear fit and also a cubic fit that is an odd function.}
\label{fig:speed_fit_lin_cubodd}
\end{minipage}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_quadratic_cubic_odd.eps}
\caption{Graph of $a_1$ and $s$ with all 3 fits (cubic fit is the odd function).}
\label{fig:speed_fit_lin_quad_cub}
\end{minipage}
\end{center}
\end{figure}

\noindent Without a doubt, for small \emph{negative} gradients ($a_1$), we get a linear relationship, generated by the line $s=-132.468a_1+0.0121156$.\\
\\
For positive gradients, it is clear that the relationship is not linear for the range of gradients we have looked at. We fitted a quadratic line to the data to give the equation $s=164802a_1^2+112.671a_1+0.00360838$. However, we believe that a cubic fit is better for our purposes. We generated 2 cubic fits - one with both even and odd terms, and the other with just odd terms. The equations of these cubics are $s=91242700a_1^3+26661.49a_1^2+166.405a_1-0.000487543$ and $s=91242700a_1^3+187.283a_1$. Of course, if $a_1$ is extremly small, we can see that there will be a linear relationship since terms of $O(a_1^2)$ can be neglected.\\
\\
There is something no quite convincing about the above results. The theory that the speed is proportional to the gradient is an established theory that has been proved. We must therefore conduct further tests in order to establish exactly why the theory does not fit our results.


\subsection{Retesting}
\label{sec:retest}

The first task we conducted was a review of the amended code. We checked that the amendments were correctly included in the code and that the code was compiling in the way that it should. Our observations could not see any errors in the code.\\
\\
However, on looking at the function that generates the initial conditions, we noticed that $a(x)$ was called. Previously, we had just $a$ which was a constant in the original code. Therefore, to elimate this as a possible cause of the discrepancy, we decided to run some tests using $a_0$ in the generation of the initial conditions rather than $a(x)=a_0+a_1x$ using various gradients. Some of our results are depicted in the figures \ref{fig:retest9x}, \ref{fig:retest9y}, \ref{fig:retest12x} and \ref{fig:retest12y}.\\

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx023.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ with original on right and retested version on left ($a_0$ for $a_1$=0.0008 in initial conditions instead of $a(x)$).}
\label{fig:retest9x}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity023.eps}
\end{minipage}
\caption{Graph of $t$ vs $y$ for $a_1$=0.0008 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest9y}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest12.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitx017.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ for $a_1$=0.0002 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest12x}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest9.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fity023.eps}
\end{minipage}
\caption{Graph of $t$ vs $y$ for $a_1$=0.0002 with original on right and retested version on left ($a_0$ in initial conditions instead of $a(x)$).}
\label{fig:retest12y}
\end{center}
\end{figure}

\noindent We can clearly see that the graphs in each figure are exactly the same and therefore we can conclude that it is qualitatively irrelevent whether we use $a_0$ (a constant) or $a(x)$ (a function evaluated at a particular $x$) to generate the initial conditions.\\
\\
Next we decided to check whether the initial conditions had an effect. There is a further theory to say that if the gradient is inverted, then the initial conditions must also be inverted. So far, the initial conditions have been the same for both positive and negative gradients. We adjusted the code yet again to take this into account and re-ran the experiments.\\
\\
We took 2 values of gradient for which the speed for the positive gradient is much greater than the speed of the negative gradient, and came up with the following results:\\

\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
Figure & $a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
Figure \ref{fig:retest13} & 0.001 & -0.0651837 & 0.264594 & 0.272504\\
Figure \ref{fig:retest14} & -0.001 & 0.065026 & -0.274845 & 0.282433\\
\hline
Figure \ref{fig:retest15} & 0.0013 & -0.119214 & 0.430456 & 0.446659\\
Figure \ref{fig:retest16} & -0.0013 & 0.124477 & -0.430456 & 0.448093\\
\hline
\end{tabular}
\label{table:speed2}
\end{center}

\noindent We can compare the results in table \ref{table:speed2} to those in the original experiments, which are shown in the following table.\\

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
0.001 & -0.0637345 & 0.262569 & 0.270194\\
-0.001 & 0.0289989 & -0.141975 & 0.144906\\
\hline
0.0013 & -0.107506 & 0.441938 & 0.454826\\
-0.0013 & 0.0.0403389 & -0.18053 & 0.184982\\
\hline
\end{tabular}
\label{table:speed3}
\end{center}

\noindent We can see that the revised figure in table \ref{table:speed3}, clearly fit the theory.\\

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest13.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest13.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=0.001}
\label{fig:retest13}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest14.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest14.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=-0.001}
\label{fig:retest14}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest15.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest15.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=0.0013}
\label{fig:retest15}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fitxretest16.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/fityretest16.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and the graph of $t$ vs $y$ on the right for $a_1$=-0.0013}
\label{fig:retest16}
\end{center}
\end{figure}

\noindent However, it is still rather puzzling as to why the original data did not fit the theory. We therefore decide to try a further test which moved the original initial conditions from its original position by a certain amount of space steps.\\
\\
Firstly, we took\\
\\
Finally, we decided to see whether the initial transient from the starting point to when the wave settles down to steady rotations has an effect on the speed of the wave. To do this we initiated a rigidly rotating wave without a gradient, letting the wave settle down and rotate about a fixed point which was as close to the centre of the box as possible. After a few rotations, the wave was stopped and the final conditions file generated by EZSpiral was used as the initial conditions file for the next few simulations. We then started EZSpiral again but this time introducing a gradient and did the usual analysis. Our results are presented in the following table \ref{table:speed4}:\\

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
$a_1$ & $\dot{x}$ & $\dot{y}$ & speed\\
\hline
-0.0014 & 0.0722856 & -0.289977 & 0.298851\\
-0.0012 & 0.0622736 & -0.239769 & 0.247724\\
-0.001 & 0.0469367 & -0.19443 & 0.200015\\
-0.0008 & 0.0353927 & -0.148323 & 0.152487\\
-0.0004 & 0.0162417 & -0.0690147 & 0.0709001\\
-0.0002 & 0.00673007 & -0.033589 & 0.0342566\\
0.0002	& -0.0076846 & 0.0330261 & 0.0339084\\
0.0004	& -0.0154812 & 0.0675423 & 0.0692938\\
0.0006 & -0.0243027 & 0.10343 & 0.106247\\
0.0008 & -0.0348249 & 0.141664 & 0.145882\\
0.001 & -0.0453209 & 0.183785 & 0.189291\\
0.0012	& -0.0544602 & 0.222769 & 0.229329\\
0.0014 & -0.0690389 & 0.277411 & 0.285873\\
0.0016 & -0.0720951 & 0.314733 & 0.322885\\
0.0018 & -0.0983964 & 0.388473 & 0.400741\\
\hline
\end{tabular}
\label{table:speed4}
\end{center}

\noindent Comparing graphically the above data we get the graphs shown in figures \ref{fig:vel_late_grad} and \ref{fig:fit_speed_late_grad}.\\


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/x_vel_late_grad.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/y_vel_late_grad.eps}
\end{minipage}
\caption{Graphs of $a_1$ vs $\dot{x}$ on the left and the graph of $a_1$ vs $\dot{y}$}
\label{fig:vel_late_grad}
\end{center}
\end{figure}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_linear_late_grad.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/initial_numerics/inhom/speed_fit_linear_cubic_odd_lategrad.eps}
\end{minipage}
\caption{Graphs of $a_1$ vs $speed$ with a linear fit on the left and a cubic fit on the right}
\label{fig:fit_speed_late_grad}
\end{center}
\end{figure}

\noindent We can see that these results now fit the theory that the speed is proportional to the gradient a lot better than in the previous cases. We can see that the fits in figure \ref{fig:fit_speed_late_grad} are very much linear fits and hence proving the theory from a numerical point of view.


\subsection{Summary for Initial Analysis}
\label{sec:summ}

We have seen that the systems studied in section \ref{sec:numanal} are sensitive to initial conditions. The initial transient before the wave settles down plays a big part in determining the speed of the wave. Therefore, in order to generate accurate results we must get rid of the initial transient by initiating a non-drifting wave that rotates around a point as close to the centre of the box as possible and then introduce a gradient to make the wave drift. This will eliminate any errors produced by the initial transient and therefore give us more accurate numerical results.

\section{Equation of motion for the tip of a rigidly rotating wave}

\subsection{setting up the equations}

Before moving on to study how drifting MRW's behave, let us consider the motion of the tip of a RW. From Biktashev 1996, we have:

\begin{eqnarray*}
\frac{\partial{\Theta}}{\partial{t}} & = & w_0\\
\frac{\partial{R}}{\partial{t}} & = & c_0e^{i\Theta}
\end{eqnarray*}

\noindent Letting $R=x(t)+iy(t)$ and $\Theta=\Theta(t)$ with $x(0)=x_0$, $y(0)=y_0$ and $\Theta(0)=\Theta_0$ gives us:

\begin{eqnarray*}
\frac{\partial{\Theta}}{\partial{t}} & = & w_0\\
\frac{\partial{x}}{\partial{t}} & = & c_0\cos(\Theta)\\
\frac{\partial{y}}{\partial{t}} & = & c_0\sin(\Theta)
\end{eqnarray*}

\noindent Solving these and letting $\frac{c_0}{w_0}=R$ yields the following solution:

\begin{eqnarray*}
\Theta & = & w_0t+\Theta_0\\
x & = & x_0+R\sin(w_0t+\Theta_0)\\
y & = & y_0-R\cos(w_0t+\Theta_0)
\end{eqnarray*}

\noindent These equations give us the equations of motion for the tip of a rigidly rotating spiral wave. A couple of steps of simple algegra produces:

\begin{eqnarray*}
(x-x_0)^2+(y-y_0)^2 & = & R
\end{eqnarray*}

\noindent which fits in with the fact that the tip of a rigidly rotating wave traces out a perfect circle.\\
\\
Earlier analysis in section \ref{sec:numanal} used $x(t)=x_0+c_xt$ and $y(t)=y_0+c_yt$ to produce a straight to determine the speed of the drifting wave. In fact, we can say that these linear equations are the actual equations of motion for the point of rotation of the drifting wave. Theresfore, we propose that the equations of motion for a rigidly rotating spiral wave that drifts are:

\begin{eqnarray*}
x & = & x_0+c_xt+R\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt-R\cos(w_0t+\Theta_0)
\end{eqnarray*}

\noindent For our purposes we now suppose that:

\begin{eqnarray*}
x & = & x_0+c_xt+R_x\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt-R_y\cos(w_0t+\Theta_0)
\end{eqnarray*}

and we should find that $R_x=R_y=R$.

\subsection{Numerical Testing of these equations}

Throughout our testing, we used Gnuplot to fit the equations to the data. However, Gnuplot is very sensitive to initial conditions and therefore we need to make a good initial estimate of what the parameters in the equations are going to be. These initial estimates, together with the results, are shown in the following subsections.

\subsubsection{y component}

Let us firstly consider fitting $y(t)$ to the $y$ component of the tip data for the gradient $a_1$=-0.0002. In order to generate a fairly accurate fitted function, we need to specify some initial hand calculated values for each of the 5 parameters. These were calculated to be:

\begin{eqnarray*}
x_0 & = & 29.9976 \\
c_x & = & -0.0336148 \\
R_x & = & 3.5 \\
\omega_x & = & 0.636809 \\
\phi_x & = & -1.37304 
\end{eqnarray*}

\noindent Firstly, it is noted that our value of $a_1$ is small and therefore the speed of the drift if also small and fits with the theory that it is linearly dependent on the gradient. Next, we conducted several fitting procedures. The first procedure used the data from just a few rotations of the wave. This was in order to see if the fitting procedure was working. The next procedure was for a few more rotations whilst the final procedure fitted the function to many rotations. Our results are shown below.

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity1.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity10.eps}
\end{minipage}
\caption{Here we fit the function over just a handful of rotations and get the function $y(t)=29.9369-0.032849t+3.5244\sin(0.636348t+0.915195)$, with $y(t)$ coinciding with the orginal trajectory on the left and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity1}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity2.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity3.eps}
\end{minipage}
\caption{The same function as in figure \ref{fig:fity1} is plotted here but the plotting on the above graphs is now over a wider range of time steps. as with figure \ref{fig:fity1}, the graph on the left has both the orginal trajectory and $y(t)$ coinciding and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity2}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity4.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity5.eps}
\end{minipage}
\caption{We now fit the function over more rotations (double the amount of the first fit) and get $y(t)=29.9519-0.0332139t+3.52898\sin(0.635567t+0.947123)$. We can see that the fitted function, $y(t)$, coincides with the orginal trajectory on the left and on the right the orginal trajectory is moved down slightly so that the curve $y(t)$ can be seen.}
\label{fig:fity3}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity6.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity7.eps}
\end{minipage}
\caption{We now fit the function over 4 times as many rotations than in the second fit shown in figure \ref{fig:fity3} above and get $y(t)=29.9864-0.0335229t+3.47646\sin(0.631333t+1.45241)$. We plot both the orginal trajectory and the fitted function, $y(t)$ over the same range and get the above graphs.}
\label{fig:fity4}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity8.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fity9.eps}
\end{minipage}
\caption{Here we keep the function found in figure \ref{fig:fity4} but plot both the original trajectory and $y(t)$ over shorter domains.}
\label{fig:fity5}
\end{center}
\end{figure}

\noindent It is clear from figures \ref{fig:fity4} and \ref{fig:fity5} that for some reason Gnuplot is not giving us accurate plots for larger domains. This could be down to the fact that because the domain is large then the plot is less accurate. Over shorter domains we get that the fitted function is almost a perfect fit. Hence to combat this, we need to adjust the accuracy in Gnuplot.

\subsubsection{x component}

Let us now do the same for the x component. The initial values are:


\begin{eqnarray*}
x_0 & = & 30.0668 \\
c_x & = & 0.00675554 \\
R_x & = & 3.51 \\
\omega_x & = & 0.636809 \\
\phi_x & = & 1.00 
\end{eqnarray*}

\noindent The results are now as follows.


\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx1.eps}
\end{minipage}
\caption{Here we fit the function over just a handful of rotations as with figure \ref{fig:fity1} and get the function $x(t)=30.1547+0.00699495t+3.52158\sin(0.63638t-2.22774)$.}
\label{fig:fitx1}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx2.eps}
\end{minipage}
\caption{The same function as in figure \ref{fig:fity1} is plotted here but the plotting on the above graphs is now over a wider range of time steps. as with figure \ref{fig:fitx1}.}
\label{fig:fitx2}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx3.eps}
\end{minipage}
\caption{We now fit the function over more rotations (double the amount of the first fit) and get $x(t)=30.1791+0.00633029t+3.52665\sin(0.635589t-2.19654)$.}
\label{fig:fitx3}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx4.eps}
\end{minipage}
\caption{We now fit the function over 4 times as many rotations than in the second fit shown in figure \ref{fig:fitx3} above and get $x(t)=30.1328+0.00642943t+3.46909\sin(0.631311t-1.68495)$.}
\label{fig:fitx4}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx5.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitx6.eps}
\end{minipage}
\caption{Here we keep the function found in figure \ref{fig:fitx4} but plot both the original trajectory and $x(t)$ over shorter domains.}
\label{fig:fitx5}
\end{center}
\end{figure}

\subsubsection{Comparing results}

Let us now compare some of the results. We should find that $R_x$ and $R_y$ are the same as should be $\omega_x$ and $\omega_y$ together with $\phi_x$ and $\phi_y$. Consider the following table.

\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Figure and component & $x_0$/$y_0$ & $c_x$/$c_y$ & $R_x$/$R_y$ & $\omega_x$/$\omega_y$ & $\phi_x$/$\phi_y$\\
\hline
Figure \ref{fig:fitx1} and x comp. & 29.9369 & -0.032849 & 3.5244 & 0.636348 & 0.915195\\
Figure \ref{fig:fity1} and y comp. & 30.1547 & 0.00699495 & 3.52158 & 0.63638 & -2.22774\\
\hline
Figure \ref{fig:fitx3} and x comp. & 29.9519 & -0.0332139 & 3.52898 & 0.635567 & 0.947123\\
Figure \ref{fig:fity3} and y comp. & 30.1791 & 0.00633029 & 3.52665 & 0.635589 & -2.19654\\
\hline
Figure \ref{fig:fitx4} and x comp. & 29.9864 & -0.0335229 & 3.47646 & 0.631333 & 1.45241\\
Figure \ref{fig:fity4} and y comp. & 30.1328 & 0.00642943 & 3.46909 & 0.631311 & -1.68495\\
\hline
\end{tabular}
\label{table:speed}
\end{center}

\noindent Clearly, $R_x$ and $R_y$ are almost the same as are $\omega_x$ and $\omega_y$. We can see that $\phi_x$ and $\phi_y$ are not the same. However, the difference between them is $\pi$ in each case. Therefore, taking the angle of the $x$-component to be $\theta$, this gives the $y$-component to be $\theta-\pi$. Hence:

\begin{eqnarray*}
\cos(\theta-\pi) & = & \cos(\theta)\cos(\pi)+\sin(\theta)\sin(\pi)\\
& = & -\cos(\theta)
\end{eqnarray*}

\noindent implying that the sign in front of cos in the equation of motion for $y$ is changed giving the folowing revised equations of motion:

\begin{eqnarray*}
x & = & x_0+c_xt+R_x\sin(w_0t+\Theta_0)\\
y & = & y_0+c_yt+R_y\cos(w_0t+\Theta_0)
\end{eqnarray*}



\section{Meandering Waves}

We have now established that EZSpiral is working correctly for rigidly rotating waves and how we should conduct future experiments. We now move on to drifting MRW's and see what results we get. Note that this area has not been touched before and the results produced are original.


subsection{Non-Drifting Meandering Waves}
We know that MRW's are quasiperiodic. Let us assume that the equations of motion are:\\

\begin{eqnarray*}
x(t) & = & x_0+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}
\\
We showed in the exercise for Rigidly Rotating waves that $R_x$ and $R_y$ are in fact the same (say $R$) as are $\omega_{1x}$ and $\omega_{1y}$ ($\omega_1$). Let us assume that $r_x$ and $r_y$ ($r$ say) are the same and also $\omega_{2x}$ and $\omega_{2y}$ are also the same ($\omega_2$). Note that $R$ and $\omega_1$ are the primary radius and primary frequency respectively, and $r$ and $\omega_2$ are the secondary radius and frequency (i.e the radius and frequency in the rotating frame of reference).\\
\\
Looking at the tip file and also at the graph of the trajectory of the wave (see figure \ref{fig:mrw41}) we get the following initial estimates of the various parameters:

\begin{eqnarray*}
x_0 & = & 28.73429 \\
y_0 & = & 28.50880 \\
R & = & 3.25 \\
\omega_1 & = & 0.162496 \\
\phi_1 & = & 1.00\\
r & = & 0.9\\
\omega_2 & = & 1.65\\
\phi_2 & = & 0.8  
\end{eqnarray*}


\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/mrw041.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/mrw041_part.eps}
\end{minipage}
\caption{Graphs of the trajectories for a non-drifting meandering wave with the full trajectory on the left and a part trajectory (1 full rotation) on the right.}
\label{fig:mrw41}
\end{center}
\end{figure}

\noindent Preliminary results using these initial estimates by Gnuplot are shown in figure \ref{fig:mrw41fit}.\\

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwy41.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwx41.eps}
\end{minipage}
\caption{Fit by Gnuplot for both $x(t)$ and $y(t)$.}
\label{fig:mrw41fit}
\end{center}
\end{figure}

\noindent It is clear that this function fits the data and the equations are given by:

\begin{eqnarray*}
x(t) & = & 30.1294+2.88181\cos(0.167468t-0.683533)+0.798711\cos(1.63341t+0.595935)\\
y(t) & = & 30.2545+2.93476\sin(0.16552t-0.597004)-0.792184\sin(1.63692t+0.437389)
\end{eqnarray*}

\noindent These functions are fitted just for 1 rotation. Let us consider more than one rotation as shown in figure \ref{fig:mrw41fitmore}.\\

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwx41more.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwy41more.eps}
\end{minipage}
\caption{Fit by Gnuplot for both $x(t)$ on the left and $y(t)$ on the right for more than 1 rotation (just over 3).}
\label{fig:mrw41fitmore}
\end{center}
\end{figure}

\noindent It is clear that this function fits the data and the equations are given by:

\begin{eqnarray*}
x(t) & = & 30.1212+2.89537\cos(0.167333t-0.674339)+0.799068\cos(1.63446t+0.544719)\\
y(t) & = & 30.356+2.9127\sin(0.167285t-0.675932)-0.794017\sin(1.63477t+0.531315)
\end{eqnarray*}

\noindent This is a more accurate fit. We can see that the parameters $R_x$, $r_x$, $\omega_{1x}$, $\omega_{2x}$, $\phi_{1x}$ and $\phi_{2x}$ to 3 signigificant figures can be said to be the same as their $y$ counterparts with the difference being less than 1\%. We conclude that for a meandering spiral wave with a stationary point of rotation we can generate the equation of the tip of the wave with the above equations.

\subsection{Drifting Meandering Wave}

We saw above that a meandering wave whose point of rotation is fixed can be approximated using the following equations:\\

\begin{eqnarray*}
x(t) & = & x_0+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}
\\
\noindent We propose that the equations of drifting meandering waves are given by:\\

\begin{eqnarray*}
x(t) & = & x_0+c_xt+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+c_yt+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}
\\
The only difference being the velocity components for $x$ and $y$. To put this proposition to the test, let us take the data for when the gradient is $a_1$=0.0004. We will use the following initial estimates of the parameters.

\begin{eqnarray*}
x_0 & = & 28.73429 \\
y_0 & = & 28.50880 \\
c_x & = & -0.00763589\\
c_y & = & -0.0104151\\
R & = & 3.25 \\
\omega_1 & = & 0.162496 \\
\phi_1 & = & 1.00\\
r & = & 0.9\\
\omega_2 & = & 1.65\\
\phi_2 & = & 0.8  
\end{eqnarray*}

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/mrw002.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/mrw002_part.eps}
\end{minipage}
\caption{Graphs of the trajectories for a drifting meandering wave with the full trajectory on the left and a part trajectory (2 full rotation) on the right.}
\label{fig:mrw002}
\end{center}
\end{figure}

\noindent We can see from figure \ref{fig:mrw002} that the wave is moving to the bottom left and actually moves rather slowly. Let us see how Gnuplot fits these functions.\\

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwx002.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/inhom/fitmrwy002.eps}
\end{minipage}
\caption{The above graphs show how the functions were fitted to the data with $x(t)$ on the left and $y(t)$ on the right.}
\label{fig:mrw002fit}
\end{center}
\end{figure}

\noindent From the graphs in figure \ref{fig:mrw002fit}, we can see that Gnuplot has fitted the functions quite well. The functions take the form:

\begin{eqnarray*}
x(t) & = & 30.4127-0.00805152t+2.91423\cos(0.166231t-0.676989)+0.795599\cos(1.63444t+0.571694)\\
y(t) & = & 29.9896-0.0107487t+2.92391\sin(0.166176t-0.666409)+0.793362\sin(1.63461t-2.59023)
\end{eqnarray*}

\subsection{Conclusion}

We can conclude from the results present in this section, that the general form of the equations of motion for the tip of a meandering wave that drifts is:

\begin{eqnarray*}
x(t) & = & x_0+c_xt+R_x\cos(\omega_{1x}t+\phi_{1x})+r_x\cos(\omega_{2x}t+\phi_{2x})\\
y(t) & = & y_0+c_yt+R_y\sin(\omega_{1y}t+\phi_{1y})-r_y\sin(\omega_{2y}t+\phi_{2y})
\end{eqnarray*}

\noindent This was shown to be true numerically and therefore we need to show it is true analytically.



==> chapter2/spiral_dynamics/initial_numerics/initial_numerics.tex <==
\section{Initial Numerical Observations and Results}

\input{chapter2/initial_numerics/inhom_numerics}
\input{chapter2/initial_numerics/resonance}
\input{chapter2/initial_numerics/report_drift_reson}

==> chapter2/spiral_dynamics/initial_numerics/report_drift_reson.tex <==
\section{Resonance - Numerical Work - pictures}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=1.0\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/traj.eps}
\end{minipage}
\caption{Meandering Spiral Wave drifting due to inhomogeneities, passing through a point of resonance.}
\label{fig:traj}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/quotient.eps}
\end{minipage}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cx_cy.eps}
\end{minipage}
\caption{The plot of the quotient system on the left and $c_x$ against $c_y$ on the right.}
\label{fig:quot}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cx_vs_om.eps}
\end{minipage}
\begin{minipage}[htbp]{0.49\linewidth}
\centering
\includegraphics[width=0.7\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/cy_vs_om.eps}
\end{minipage}
\caption{$c_x$ against $\omega$ on the left and $c_y$ against $\omega$ on the right.}
\label{fig:quot1}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=1.0\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/speed.eps}
\end{minipage}
\caption{$\frac{dx}{dt}$ versus $\frac{dy}{dt}$.}
\label{fig:speed}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[htbp]{0.7\linewidth}
\centering
\includegraphics[width=1.0\textwidth, angle=-90]{chapter2/initial_numerics/picsrdr/poincare_0.008.eps}
\end{minipage}
\caption{The Poincare Cross Section. Time is plotted on the horizontal axis and $y$ on the vertical.}
\label{fig:pcs}
\end{center}
\end{figure}


==> chapter2/spiral_dynamics/initial_numerics/resonance.tex <==
\section{Behaviour around a point of resonance}

\subsection{Introduction}
\label{ch:intro}

In this analysis we look at how the meandering spiral wave behaves near points of resonances when we induce the wave to drift by applying a gradient. Meandering spiral waves are quasiperiodic solutions to the governing equations and therefore we must have that the two frequencies are not rationally related, i.e.
\[\frac{\omega_1}{\omega_2} \neq \frac{p}{q} \hfill \mbox{ s.t. } p,q \in \mathbb{Z}\]
We find however that we come across frequencies that are almost rationally related but not quite, and the parameters for which this occurs give us the point of resonance.\\
\\
In this analysis, we will take the parameters $a_0=0.01875$, $b=0.01$ and $\epsilon =0.01$, which almost gives us a 4:1 resonance, i.e. the secondary frequency is 4 times that of the primary frequency (the actual ratio is approximately 4.027:1).

\subsection{Initial Analysis}

As usual, we have kept the parameters $a_0$ and $\epsilon$ fixed and vary the gradient, $a_1$. We also use the technique developed previous reports whereby we initate the wave with the centre of rotation as close to the centre of the domain as possible. We display the initial trajectories in Figs. \ref{fig:mrwres001} to \ref{fig:mrwres015}, with the trajectory in Fig. \ref{fig:mrwres001} being the meandering spiral wave with no gradient applied and therefore it does not drift. Also, in Fig. \ref{fig:mrwres001} we have include just 2 full rotations and it can been seen on closer inspection that there are almost exactly 4 inward facing ``petals" corresponding to the 4:1 resonance.\\
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres001.eps}
\caption{$a_1=0$}
\label{fig:mrwres001}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres002.eps}
\caption{$a_1=0.0002$}
\label{fig:mrwres002}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres003.eps}
\caption{$a_1=0.0004$}
\label{fig:mrwres003}
\end{minipage}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres004.eps}
\caption{$a_1=0.0006$}
\label{fig:mrwres004}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres005.eps}
\caption{$a_1=0.0008$}
\label{fig:mrwres005}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres006.eps}
\caption{$a_1=0.001$}
\label{fig:mrwres006}
\end{minipage}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres007.eps}
\caption{$a_1=0.0012$}
\label{fig:mrwres007}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres008.eps}
\caption{$a_1=0.0014$}
\label{fig:mrwres008}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres009.eps}
\caption{$a_1=-0.0002$}
\label{fig:mrwres009}
\end{minipage}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres010.eps}
\caption{$a_1=-0.0004$}
\label{fig:mrwres010}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres011.eps}
\caption{$a_1=-0.0006$}
\label{fig:mrwres011}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres012.eps}
\caption{$a_1=0.0008$}
\label{fig:mrwres012}
\end{minipage}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres013.eps}
\caption{$a_1=-0.001$}
\label{fig:mrwres0013}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres014.eps}
\caption{$a_1=-0.0012$}
\label{fig:mrwres014}
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres015.eps}
\caption{$a_1=-0.0014$}
\label{fig:mrwres015}
\end{minipage}
\end{center}
\end{figure}
\\
Initial observations show that near a point of resonance, the spiral wave does not behave like what we have previously observed in other numerical experiments. We can see from Fig. \ref{fig:mrwres002} that the wave almost looks as though it behaves like a Rigidly Rotating spiral wave for the first part of the trajectory but in fact on closer inspection we can see that the trajectory slightly oscilates from side to side as it progresses, which is due to the presence of the secondary frequency.\\
\\
Then, as the wave reaches a certain point, it's trajectory changes. We have split up this trajectory to demonstrate this behaviour in more detail and this is shown in Figs. \ref{fig:reson2} to \ref{fig:reson5}.
\\
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/reson2.eps}
\caption{The first part of the trajectory for $a_1=0.0002$.}
\label{fig:reson2}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/reson3.eps}
\caption{The last part of the trajectory for $a_1=0.0002$}
\label{fig:reson3}
\end{minipage}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/reson4.eps}
\caption{A few rotations of the wave as we just get into the last part of the trajectory for $a_1=0.0002$.}
\label{fig:reson4}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/reson5.eps}
\caption{As for Fig. \ref{fig:reson4} but with more rotations.}
\label{fig:reson5}
\end{minipage}
\end{center}
\end{figure}
\\
As we can see, once the wave reaches this particular point, the meandering motion of the wave is greatly exagerated and also the wave changes direction. As we increase the gradient, $a_1$, we can see that this phenominem changes - the direction of motion changes, the severity of the change of motion also changes.\\
\\
Once we reach a certain value of the gradient, it can be seen that we no longer get this phenominem but the spiral wave drifts out of the domain. Also, as the gradient increases, the direction of travel also increases. Whether this change is proportional to the gradient has yet to be investigated. Also, for $a_1=\pm 0.0014$, we observe that the trajectory generated is very strange. This appears to be due to the fact that in this particular instance the gradient is too large. Again, further investigation is needed.\\
\\
Furthermore, for $a_1=\pm 0.0004$, the trajectory of the wave looks as though it bends to the right for the positive value and to the left for the negative value. Further investigation is also needed in this instance.\\
\\
Initially, we thought that the boudaries may have an affect and cause the phenominem described above. Therefore, we ran the experiment in a larger domain for $a_1=0.0002$ ($L_x$ was now to be increased from 60 to 120 and the number of points, $N_x$, increased from 181 to 361 - therefore the space step was kept constant). We can see from Fig. \ref{fig:mrwres016}, that the same phenominem occurs. The trajectory begins as in the smaller domain, looking as though it is moving like a Rigidly Rotating wave. Then once it gets to a certain point, it changes direction and the trajectory gets wider. This is as per the smaller domain, so therefore we can say that the phenominem may not depend on the domain size and nor does the boundary have an influence.\\
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.75\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwres016.eps}
\caption{Trajectory of the spiral wave for $a_1$=0.0002 in a larger domain.}
\label{fig:mrwres016}
\end{minipage}

\end{center}
\end{figure}
\\
Finally, we show the tajectories for both time against $x$ and also time against $y$ in Figs. \ref{fig:mrwresx002} and \ref{fig:mrwresy002}. Clearly, when the trajectory reaches a particular point, it changes direction and shape. It looks as though the primary radius (i.e. the radius of the circle in the absence of the secondary frequency) has actually increased. This needs to be looked at in more detail together with whether the speed of the wave is proportional to the gradient as per previous analysis.\\
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwresx002.eps}
\caption{Time against $x$ for $a_1=0.0002$.}
\label{fig:mrwresx002}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/initial_numerics/resonance1/mrwresy002.eps}
\caption{Time against $y$ for $a_1=0.0002$.}
\label{fig:mrwresy002}
\end{minipage}
\end{center}
\end{figure}

\subsection{Brief Summary}

To conclude this brief report we can summarise as follows:\\
\\
$\bullet$ For small gradients there are points at which the trajectory of the wave changes.\\
$\bullet$ For different values of the gradient, we get the wave travelling in different directions.\\
$\bullet$ For large gradient, we do not observe the phenominem seen for small gradients.\\
$\bullet$ Initial observations suggest that the boundaries are not responsible for this phenominem.\\
\\
Further investigation is needed on the following.\\
\\
$\bullet$ Is the direction of the wave for various gradients proportional to the gradient?\\
$\bullet$ At what point does the observed phenominem cease?\\
$\bullet$ Various other parameter ($a_0$ and $b$) needed to investigated to see if there are so called "tongues" in which this phenominem occurs.\\
$\bullet$ What is the maximum gradient that can be applied in this instance to get a meaningful result and is this dependent on the other parameters?\\
$\bullet$ Why does the trajectory curve to the right (left) for $a_1$=0.0004(=-0.0004)?\\
$\bullet$ Is the speed of the wave proportional to the gradient?\\
$\bullet$ How does the primary radius change and to what extent does it change for various gradients?

==> chapter2/spiral_waves/ODEsolve.tex <==
\subsection{Solution to the ODE system}

\subsubsection{Analysis}
The following system is taken from the 1996 paper by Biktashev et al regarding Meander of Spiral Waves and Symmetry of the Plane~\cite{Bik96}:\\
\begin{eqnarray}
\label{eqn:dotx}
\dot{x} & = & s(t)\cos(\theta(t))\\
\label{eqn:doty}
\dot{y} & = & s(t)\sin(\theta(t))\\
\label{eqn:dottheta}
\dot{\theta} & = & \omega(t)\\
\label{eqn:dots}
\dot{s} & = & F(s,w)\\
\label{eqn:dotomega}
\dot{\omega} & = & G(s,w)
\end{eqnarray}
\\
In this system, $(x,y)$ are the coordinates of the tip of the wave, $s(t)$ represents the speed, $\theta(t)$ is the angle of rotation with respect to the $x$-axis, and $\omega$ is the frequency of the wave. Various authors have documented the observation that the transition from Rigid Rotation to Meander of the Spiral Wave is via a Hopf Bifurcation. We therefore exploit this fact in the following analysis, i.e. we are seeking limit cycle solutions.\\
\\
In the system above, the bifurcation parameters are $s$ and $\omega$. Therefore, the Hopf Bifurcation must be contained in equations (\ref{eqn:dots}) and (\ref{eqn:dotomega}) of the above system. The normal form of the Hopf Bifurcation~\cite{kuznetsov} is:\\
\begin{equation}
\label{eqn:normal}
\dot{z} = \alpha  'z-\beta ' z|z|^2
\end{equation}
\\
where $\alpha '=a_1+ia_2$, $\beta '=b_1+ib_2$ and $z\in\mathbb{C}$. A limit cycle solution to this equation is of the form:\\
\begin{equation}
\label{eqn:limcyc}
z = re^{i\beta}
\end{equation}
\\
where $\beta=\nu t+\phi$, and the constants $r,\nu, \phi \in \mathbb{R}$. In this case, $\nu$ is the hopf frequency. Substituting (\ref{eqn:limcyc}) into (\ref{eqn:normal}), gives us:\\
\begin{eqnarray*}
i\nu r e^{i\beta} & = & \alpha ' re^{i\beta}-\beta ' r^3e^{i\beta}\\
\Rightarrow i\nu r & = & \alpha ' r-\beta ' r^3\\
\Rightarrow i\nu r & = & (a_1+ia_2)r-(b_1+ib_2)r^3
\end{eqnarray*}
\\
Equating real and imaginary parts, we get:
\begin{equation}
\label{eqn:r}
r = \sqrt{\frac{a_1}{b_1}}
\end{equation}
\begin{equation}
\label{eqn:nu}
\nu = \frac{a_2b_1-b_2a_1}{b_1}
\end{equation}\\
We now let $s=s(z)$ and $\omega=\omega(z)$~\cite{Bik96}:\\
\begin{eqnarray}
\label{eqn:s}
s & = & s_0+s_1z+\bar{s}_1\bar{z}+\mbox{h.o.t.}\\
\label{eqn:omega}
\omega & = & \omega_0+\omega_1z+\bar{\omega}_1\bar{z}+\mbox{h.o.t.}
\end{eqnarray}\\
where, the bar represents the complex conjugate and $\omega_0\in\mathbb{R}$, $\omega_1\in\mathbb{C}$. Let us consider $\omega(z)$. Substituting (\ref{eqn:limcyc}) into (\ref{eqn:omega}), letting $\omega_1=\omega_{11}+i\omega_{12}$ and discarding higher order terms (h.o.t.), we get:\\
\begin{eqnarray}
\omega & = & \omega_0+\omega_1re^{i\beta}+\bar{\omega}_1re^{-i\beta}\\
\Rightarrow \omega & = & \omega_0+r(\omega_1e^{i\beta}+\bar{\omega}_1e^{-i\beta})
\end{eqnarray}\\
From (\ref{eqn:dottheta}), we get that:\\
\begin{eqnarray}
\dot{\theta} & = & \omega(t)\\
\Rightarrow \theta(t) & = & \int{\omega(t)}dt\\
\Rightarrow \theta(t) & = & \int{(\omega_0+r(\omega_1e^{i\beta}+\bar{\omega}_1e^{-i\beta}))}dt\\
\Rightarrow \theta(t) & = & \theta_0+\omega_0t-i\frac{\omega_1r}{\nu}e^{i\beta}+i\frac{\bar{\omega}_1r}{\nu}e^{-i\beta}
\end{eqnarray}\\
Also, we have that:\\
\begin{equation}
s(t) = s_0+s_1re^{i\beta}+\bar{s}_1re^{-i\beta}
\end{equation}\\
Now (\ref{eqn:dotx}) and (\ref{eqn:doty}) imply that:\\
\begin{eqnarray}
\dot{x}+i\dot{y} & = & s(t)e^{i\theta(t)}\\
\Rightarrow \dot{x}+i\dot{y} & = & (s_0+s_1re^{i\beta}+\bar{s}_1re^{-i\beta})e^{i(\theta_0+\omega_0t-i\frac{\omega_1r}{\nu}e^{i\beta}+i\frac{\bar{\omega}_1r}{\nu}e^{-i\beta})}\\
\Rightarrow \dot{x}+i\dot{y} & = & (s_0+s_1re^{i\beta}+\bar{s}_1re^{-i\beta})e^{i(\theta_0+\omega_0t)}e^{(\frac{\omega_1r}{\nu}e^{i\beta}-\frac{\bar{\omega}_1r}{\nu}e^{-i\beta})}\\
\label{eqn:xdotydot}
\Rightarrow \dot{x}+i\dot{y} & = & (s_0+s_1re^{i\beta}+\bar{s}_1re^{-i\beta})e^{i\alpha}e^{\frac{r}{\nu}(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta})}
\end{eqnarray}\\
where $\alpha=\omega_0t+\theta_0$. It is clear that we now have exponentials contained in exponentials and therefore we need to eliminate this. We note that since $r$ is small, we can expand the exponential to first order:\\
\begin{equation}
e^{\frac{r}{\nu}(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta})} = 1+\frac{r}{\nu}(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta})+O(r^2)
\end{equation}\\
Therefore, Eqn. (\ref{eqn:xdotydot}) now becomes:\\
\begin{eqnarray}
\dot{x}+i\dot{y} & = & (s_0+s_1re^{i\beta}+\bar{s}_1re^{-i\beta})e^{i\alpha}(1+\frac{r}{\nu}(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta}))\\
& = & e^{i\alpha}(s_0+r(s_1+\frac{s_0}{\nu}\omega_1)e^{i\beta}+r(\bar{s}_1-\frac{s_0}{\nu}\bar{\omega}_1)e^{-i\beta})+O(r^2)
\end{eqnarray}\\
We now integrate with respect to $t$ to get:\\
\begin{eqnarray*}
x+iy &=& (x_0+iy_0)-i\frac{s_0}{\omega_0}e^{i\alpha}-i e^{i\alpha}\left(\frac{r}{\nu+\omega_0}(s_1+\frac{s_0}{\nu}\omega_1)e^{i\beta}-\frac{r}{\nu-\omega_0}(\bar{s}_1-\frac{s_0}{\nu}\bar{\omega}_1)e^{-i\beta}\right)\\
&=& (x_0+iy_0)-i\frac{s_0}{\omega_0}e^{i\alpha}\\
&& -i e^{i\alpha}\frac{r}{\nu(\nu^2-\omega_0^2)}\left((\nu s_1+s_0\omega_1)(\nu-\omega_0)e^{i\beta}-(\nu\bar{s}_1-s_0\bar{\omega}_1)(\nu+\omega_0)e^{-i\beta}\right)
\end{eqnarray*}\\
Therefore, we have:\\
\begin{equation}
\label{eqn:solxy}
\boxed{x+iy = x_0+iy_0-iRe^{i\alpha}-A'ie^{i\alpha}\left(Be^{i\beta}-Ce^{-i\beta}\right)}
\end{equation}\\
where:\\
\begin{eqnarray*}
R &=& \frac{s_0}{\omega_0}\\
A' &=& \frac{r}{\nu(\nu^2-\omega_0^2)}\\
B &=& (\nu s_1+s_0\omega_1)(\nu-\omega_0)\\
C &=& (\nu\bar{s}_1-s_0\bar{\omega}_1)(\nu+\omega_0)
\end{eqnarray*}\\
Consider $B$ and $C$ for a moment. \\
\begin{eqnarray}
B &=& (\nu s_1+s_0\omega_1)(\nu-\omega_0)\\
\label{eqn:B}
&=& \nu(\nu-\omega_0)s_1+s_0(\nu-\omega_0)\omega_1
\end{eqnarray}\\
Similarly for $C$:\\
\begin{eqnarray}
C &=& (\nu\bar{s}_1-s_0\bar{\omega}_1)(\nu+\omega_0)\\
\label{eqn:C}
&=& \nu(\nu+\omega_0)\bar{s}_1-s_0(\nu+\omega_0)\bar{\omega}_1
\end{eqnarray}\\
Substituting Eqns. (\ref{eqn:B}) and (\ref{eqn:C})  into (\ref{eqn:solxy}) and rearranging, we get:\\
\begin{eqnarray*}
x+iy &=& x_0+iy_0-iRe^{i\alpha}-A'ie^{i\alpha}\left(\nu^2(s_1e^{i\beta}-\bar{s}_1e^{-i\beta})+\nu s_0(\omega_1e^{i\beta}+\bar{\omega}_1e^{-i\beta})\right.\\
&& \left. -\nu\omega_0(s_1e^{i\beta}+\bar{s}_1e^{-i\beta})-\omega_0s_0(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta})\right)
\end{eqnarray*}\\
Using $s_1=s_{11}+is_{12}$ and $\omega_1=\omega_{11}+i\omega_{12}$ we have that:\\
\begin{eqnarray}
(s_1e^{i\beta}+\bar{s}_1e^{-i\beta}) &=& 2s_{11}\cos(\beta)-2s_{12}\sin(\beta)\\
(s_1e^{i\beta}-\bar{s}_1e^{-i\beta}) &=& 2is_{11}\sin(\beta)+2is_{12}\cos(\beta)\\
(\omega_1e^{i\beta}+\bar{\omega}_1e^{-i\beta}) &=& 2\omega_{11}\cos(\beta)-2\omega_{12}\sin(\beta)\\
(\omega_1e^{i\beta}-\bar{\omega}_1e^{-i\beta}) &=& 2i\omega_{11}\sin(\beta)+2i\omega_{12}\cos(\beta)
\end{eqnarray}\\
Therefore, we now have:\\
\begin{eqnarray*}
x+iy &=& x_0+iy_0-iRe^{i\alpha}-A'ie^{i\alpha}\left(2\nu^2i(s_{11}\sin(\beta)+s_{12}\cos(\beta))+2\nu s_0(\omega_{11}\cos(\beta)-\omega_{12}\sin(\beta))\right.\\
&& \left.-2\nu\omega_0(s_{11}\cos(\beta)-s_{12}\sin(\beta))-2i\omega_0 s_0(\omega_{11}\sin(\beta)+\omega_{12}\cos(\beta))\right)\\
&=& x_0+iy_0-iRe^{i\alpha}-A'ie^{i\alpha}\left(2i(\nu^2s_{11}-\omega_0s_0\omega_{11})\sin(\beta)+2i(\nu^2s_{12}-\omega_0s_0\omega_{12})\cos(\beta)\right.\\
&& \left.+2\nu(s_0\omega_{11}-\omega_0s_{11})\cos(\beta)-2\nu(s_0\omega_{12}-\omega_0s_{12})\sin(\beta)\right)
\end{eqnarray*}\\
Let $M=m_1+im_2$ and $N=n_1+in_2$ where:\\
\begin{eqnarray*}
m_1 &=& \nu^2s_{11}-\omega_0s_0\omega_{11}\\
m_2 &=& \nu(s_0\omega_{12}-\omega_0s_{12})\\
n_1 &=& \nu(s_0\omega_{11}-\omega_0s_{11})\\
n_2 &=& \nu^2s_{12}-\omega_0s_0\omega_{12}
\end{eqnarray*}\\
Therefore, we get another form of the solution as:\\
\begin{equation}
\label{eqn:solxy2}
\boxed{x+iy = x_0+iy_0-iRe^{i\alpha}+Ae^{i\alpha}(M\sin(\beta)-iN\cos(\beta))}
\end{equation}\\
where $A=\frac{2r}{\nu(\nu^2-\omega_0^2)}$. Furthermore, we can put Eqn. (\ref{eqn:solxy2}) into trigonometric terms as follows:\\
\begin{eqnarray*}
x+iy &=& x_0+iy_0-iRe^{i\alpha}+Ae^{i\alpha}((m_1+im_2)\sin(\beta)-i(n_1+in_2)\cos(\beta))\\
\left(\begin{array}{c}x\\y \end{array}\right) &=& \left(\begin{array}{c}x_0\\y_0 \end{array}\right)+R\left(\begin{array}{c}\sin(\alpha)\\-\cos(\alpha) \end{array}\right)\\
&& +A((m_1\sin(\beta)+n_2\cos(\beta))+i(m_2\sin(\beta)-n_1\cos(\beta)))\left(\begin{array}{c}\cos(\alpha)\\\sin(\alpha) \end{array}\right)\\
&=& \left(\begin{array}{c}x_0\\y_0 \end{array}\right)+R\left(\begin{array}{c}\sin(\alpha)\\-\cos(\alpha) \end{array}\right)+A[(m_1\sin(\beta)+n_2\cos(\beta))\cos(\alpha)-(m_2\sin(\beta)-n_1\cos(\beta))\sin(\alpha)\\
&& +i(m_2\sin(\beta)-n_2\cos(\beta)\cos(\alpha)+i(m_1\sin(\beta)+n_2\cos(\beta))\sin(\alpha))]
\end{eqnarray*}\\
which can be represented in the following form:\\
\begin{equation}
\label{eqn:soltrig}
\boxed{\left(\begin{array}{c}x\\y \end{array}\right) = \left(\begin{array}{c}x_0\\y_0 \end{array}\right)+R\left(\begin{array}{c}\sin(\alpha)\\-\cos(\alpha) \end{array}\right)+A
\left(\begin{array}{cc}\cos(\alpha) & -\sin(\alpha)\\ \sin(\alpha) & \cos(\alpha) \end{array}\right)\left(\begin{array}{c} m_1\sin(\beta)+n_2\cos(\beta) \\ m_2\sin(\beta)-n_1\cos(\beta) \end{array}\right)}
\end{equation}\\
The solution in the form shown in Eqn. (\ref{eqn:soltrig}) is, in our opinion, easier to use when fitting the solution to the original 5 dimensional ODE system to numerical data, as it is clear what $x(t)$ and $y(t)$ are form this equation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Summary}

Let us just summerise our results:
\subsubsection{Solution 1}
\begin{equation}
x+iy = x_0+iy_0-iRe^{i\alpha}-A'ie^{i\alpha}\left(Be^{i\beta}-Ce^{-i\beta}\right)
\end{equation}
\begin{eqnarray}
\alpha &=& \omega_0t+\theta_0\\
\beta &=& \nu t+\phi\\
A' &=& \frac{r}{\nu(\nu^2-\omega_0^2)}\\
B &=& (\nu s_1+s_0\omega_1)(\nu-\omega_0)\\
C &=& (\nu\bar{s}_1-s_0\bar{\omega}_1)(\nu+\omega_0)\\
R &=& \frac{s_0}{\omega_0}
\end{eqnarray}

\subsubsection{Solution 2}
\begin{equation}
x+iy = x_0+iy_0-iRe^{i\alpha}+Ae^{i\alpha}(M\sin(\beta)-iN\cos(\beta))
\end{equation}
where $\alpha$ and $\beta$ are as per Solution 1 and:
\begin{eqnarray}
A &=& \frac{2r}{\nu(\nu^2-\omega_0^2)}\\
M &=& m_1+im_2\\
N &=& n_1+in_2\\
m_1 &=& \nu^2s_{11}-\omega_0s_0\omega_{11}\\
m_2 &=& \nu(s_0\omega_{12}-\omega_0s_{12})\\
n_1 &=& \nu(s_0\omega_{11}-\omega_0s_{11})\\
n_2 &=& \nu^2s_{12}-\omega_0s_0\omega_{12}
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Solution 3}

\begin{equation}
\left(\begin{array}{c}x\\y \end{array}\right) = \left(\begin{array}{c}x_0\\y_0 \end{array}\right)+R\left(\begin{array}{c}\sin(\alpha)\\-\cos(\alpha) \end{array}\right)+A
\left(\begin{array}{cc}\cos(\alpha) & -\sin(\alpha)\\ \sin(\alpha) & \cos(\alpha) \end{array}\right)\left(\begin{array}{c} m_1\sin(\beta)+n_2\cos(\beta) \\ m_2\sin(\beta)-n_1\cos(\beta) \end{array}\right)
\end{equation}
where $\alpha$, $\beta$, $R$, $A$, $m_1$, $m_2$, $n_1$, and $n_2$ are as solutions 1 and 2 above.





==> chapter2/spiral_waves/fit_ODEsolve_data.tex <==
\subsection{Fit Data}

\subsubsection{Introduction}

In our previous report, we produced an analytical solution to the five dimensional system of ODE's, which are reproduced below:

\begin{eqnarray}
\label{eqn:dotx}
\dot{x} & = & s(t)\cos(\theta(t))\\
\label{eqn:doty}
\dot{y} & = & s(t)\sin(\theta(t))\\
\label{eqn:dottheta}
\dot{\theta} & = & \omega(t)\\
\label{eqn:dots}
\dot{s} & = & F(s,w)\\
\label{eqn:dotomega}
\dot{\omega} & = & G(s,w)
\end{eqnarray}

The solution to the above system was found to be:

\begin{equation}
\label{eqn:sol}
x+iy = x_0+iy_0+e^{i\tilde{\alpha}}(C+\tilde{D}e^{i\tilde{\beta}}+\tilde{E}e^{-i\tilde{\beta}})
\end{equation}
\\
where:

\begin{eqnarray*}
\tilde{\alpha} &=& (\omega_0t+\theta_0)+(\frac{2r\omega_{11}}{\nu})(\nu t+\phi)+2ir\omega_{12}-\frac{\pi}{2}\\ 
\tilde{\beta} &=& \nu t+\phi+\tan^{-1}(\frac{s_{12}}{s_{11}})
\end{eqnarray*} 

\[\begin{array}{rclcrcl}
(x_0,y_0) &=& (x(0),y(0)) & , & C &=& \frac{s_0}{\omega_0+2r\omega_{11}}\\
\tilde{D} &=& \frac{r\sqrt{s_{11}^2+s_{12}^2}}{\omega_0+\nu+2r\omega_{11}} & , & \tilde{E} &=& \frac{r\sqrt{s_{11}^2+s_{12}^2}}{\omega_0-\nu+2r\omega_{11}}
\end{array}\]

Now, we note from Eqns. (\ref{eqn:dotx}) and (\ref{eqn:doty}) that:

\begin{eqnarray}
s(t) &=& \sqrt{\dot{x}^2+\dot{y}^2}\\
\theta(t) &=& \tan^{-1}\left(\frac{\dot{y}}{\dot{x}}\right)
\end{eqnarray}

Using the data from the tip files produced by EZSpiral, we can calculate $\dot{x}$ and $\dot{y}$, and hence $s(t)$, $\theta(t)$ and therefore $\omega(t)$ (from Eqn. (\ref{eqn:dottheta})). Next, we note that $s(t)$ and $\omega(t)$ have the following forms:

\begin{eqnarray}
\omega & = & \omega_0+\omega_1re^{i\beta}+\bar{\omega}_1re^{-i\beta}\\
\Rightarrow \omega & = & \omega_0+r(\omega_1e^{i\beta}+\bar{\omega}_1e^{-i\beta})
\end{eqnarray}

Hence, we can then fit the above functions to the numerical values of $s(t)$ and $\omega(t)$, thereby determining the coefficients and solution to the ODE system - i.e. fit the function in Eqn. (\ref{eqn:sol}) to the orginal trajectory drawn from the tip file.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Results}
Before trying to fit the results, let us see what we are trying to fit the functions to. Fig. (\ref{fig:traj}) shows the full trajectory with the parameter values $a_0=0.6$ and $b=0.115$. Also note that the numerical parameters have values $L_{x,y}=30$, $N_{x,y}=211$ and the number of steps per plot was 1. The space step is $h_x=\frac{1}{7}$ and the time step is $h_t=\frac{3}{490}$. It is clear that the wave is a inward meandering spiral, and also the parameter coordinates lie close to the Hopf Locus separating rigid rotation from meandering. Also, we have shown what the trajectories of $t$ vs $x$ and $t$ vs $y$ looks like, as we will be fitting these separately later on in the report.

\begin{figure}[tbp]
\begin{center}
\begin{minipage}[b]{0.6\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/traj.eps}
\end{minipage}
\caption{Trajectory for $a_0=0.6$ and $b=0.115$.}
\label{fig:traj}
\end{center}
\end{figure}
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/tvx.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/tvy.eps}
\end{minipage}
\caption{Graph of $t$ vs $x$ on the left and $t$ vs $y$ on the right.}
\label{fig:tvxy}
\end{center}
\end{figure}

In the following subsections, we present the results from the three different types of numerical differentiation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Method 1}

In this section, we use the following formula for calculating the numerical differentiation of our data:

\begin{equation}
\label{eqn:meth1}
\left.\frac{dx}{dt}\right |_{t_2} = \frac{x_2-x_1}{t_2-t_1}
\end{equation}

We compiled a simple C code that calculated $\left.\frac{dx}{dt}\right |_{t_i}$, $\left.\frac{dy}{dt}\right |_{t_i}$, $s(t_i)$, $\omega(t_i)$ and $\theta(t_i)$, and then wrote their values to a data file. The information in this data file was then manipulated using Gnuplot to produce various figures.

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/s_v1.eps}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/s_v1_close.eps}
\end{minipage}
\caption{Graph of $t$ vs $s(t)$ on the left. On the right is a smaller segment of the graph on the left.}
\label{fig:sver1}
\end{center}
\end{figure}

The first figure is Fig. (\ref{fig:sver1}). As we can see, there looks as though there is a quasiperiodic nature to this curve. In Fig. (\ref{fig:sver1smooth}), we have instructed Gnuplot to fit a smooth curve to this otherwise rugged looking curve. This seems to fit in to what we are looking for.\\

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.6\linewidth}
\centering
\includegraphics[width=1.3\textwidth]{chapter2/Spiral_waves/fit_ODEsolve_data/s_v1_smooth.eps}
\end{minipage}
\caption{Graph of $t$ vs $s(t)$ with a smooth curve fitted to the data.}
\label{fig:sver1smooth}
\end{center}
\end{figure}

Let us for a minute consider what form $s(t)$ and $\omega(t)$ take. If $z$ is our limit cycle solution, $z=re^{i(\nu t+\phi)}$, then $s(t)$ and $\omega(t)$ will be functions of $z$:

\begin{eqnarray}
s(t) &=& s_0+s_1z+\bar{s}_1\bar{z}+\mbox{h.o.t.}\\
\omega(t) &=& \omega_0+\omega_1z+\bar{\omega}_1\bar{z}+\mbox{h.o.t.}\\
\Rightarrow s(t) &=& s_0+s_1re^{i(\nu t+\phi)}+\bar{s}_1re^{-i(\nu t+\phi)}+\mbox{h.o.t.}\\
\Rightarrow \omega(t) &=& \omega_0+\omega_1re^{i(\nu t+\phi)}+\bar{\omega}_1re^{-i(\nu t+\phi)}+\mbox{h.o.t.}
\end{eqnarray}

If we let $s_1=s_{11}+is_{12}$ and $\omega_1=\omega_{11}+i\omega_{12}$ then we get:

\begin{eqnarray}
s(t) &=& s_0+2s_{11}r\cos(\nu t+\phi)-2s_{12}r\sin(\nu t+\phi)\\
\omega(t) &=& \omega_0+2\omega_{11}r\cos(\nu t+\phi)-2\omega_{12}r\sin(\nu t+\phi)\\
\Rightarrow s(t) &=& s_0+A\cos(\nu t+\phi)-B\sin(\nu t+\phi)\\
\Rightarrow \omega(t) &=& \omega_0+C\cos(\nu t+\phi)-D\sin(\nu t+\phi)
\end{eqnarray}

for some constants $A$, $B$, $C$, and $D$. Once we have determined these constants together with $s_0$, $\omega_0$, $\nu$ and $\phi$, we can then find the other constants $s_{11}$, $s_{12}$, $\omega_{11}$ and $\omega_{12}$, and substitute these into Eqn. (\ref{eqn:sol}) to find what the the equation of motion will be.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Method 2}

We use the following formula for calculating the numerical differentiation of our data:

\begin{equation}
\label{eqn:meth2}
\left.\frac{dx}{dt}\right|_{t_2} = \frac{x_3-x_1}{t_3-t_1}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Method 3}

We use the following formula for calculating the numerical differentiation of our data:

\begin{equation}
\label{eqn:meth3}
\left.\frac{dx}{dt}\right |_{t_3} = \frac{-x_5+8x_4-8x_2+x_1}{3(t_5-t_1)}
\end{equation}


==> chapter2/spiral_waves/spiral_waves.tex <==
\section{Introduction To Spiral Waves}

Spirals occur right throughout Nature. From Spiral Galaxies that are many 
millions of light years in diameter, to snail shells that are maybe only a 
centimetre or two across. From Hurricanes to the pattern formation of 
sunflower seeds. One important occurance of spirals in Nature that, over the 
last 30 years, has been the subject of intensive research, is the appearence 
of Spiral Wave patterns in Cardiac Models, and in particular Spiral Waves 
have been largely linked to the onset of Cardiac Arrythmias. Hence, the 
study of the onset of these Spiral Waves and how they behave is an area of 
research that has attracted a lot of attention over the years. In this 
project, we produce a study of a particular type of motion of the Spiral 
Wave, Meander.

Many models of Cardiac Excitation have been produced, most notably 
Hodgkin-Huxley (1952) and the Fitzhugh-Nagumo (1961). Many studies have been 
conducted on these models and further models have been devised on the basis 
of these studies. Back in the early 1990's, Dwight Barkley, a Mathematician 
now based at Warwick University, England, devised a model that allowed for 
fast computer similuation of waves in excitable media \cite{Bark91}. The model in 
question is a simplified version of the Fitzhugh-Nagumo model (FHN) and is 
given as follows:

\begin{eqnarray*}
\frac{\partial{u}}{\partial{t}} & = & f(u,v)+\nabla^2u\\
\frac{\partial{v}}{\partial{t}} & = & g(u,v)
\end{eqnarray*}
\\
with the local kinetics given by:

\begin{eqnarray*}
f(u,v) & = & \epsilon^{-1}u(1-u)[u-u_{th}(v)]\\
g(u,v) & = & u-v
\end{eqnarray*}
\\
where $u_{th}(v)=(v+b)/a$ and $a, b$, and $\epsilon$ are parameters.

The model introduced by Barkley was shown, under certain conditions, to 
behave in a similar manner to that of the FHN model, but was far simplier to 
study from a numerical point of view. It has been shown by Barkley himself 
that the model can produce waves that meander. This report will bring 
together the basic properties of this particular motion and will show how 
numerical simulations can be used to generate meandering waves by using a 
program called EZSpiral. Further, we will also introduce some interesting 
results that will hopefully be the subject of further investigation.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Barkley's Model}

As shown in the Introduction, Barkley's model is given by:
\begin{eqnarray*}
\frac{\partial{u}}{\partial{t}} & = & f(u,v)+\nabla^2u\\
\frac{\partial{v}}{\partial{t}} & = & g(u,v)
\end{eqnarray*}
\\
with the local kinetics given by:

\begin{eqnarray*}
f(u,v) & = & \epsilon^{-1}u(1-u)[u-u_{th}(v)]\\
g(u,v) & = & u-v
\end{eqnarray*}

where $u_{th}(v)=(v+b)/a$ and $a, b$, and $\epsilon$ are parameters. This 
model is a simplified version of the FHN model, which is stated below:

\begin{eqnarray*}
\frac{\partial{u}}{\partial{t}} & = & f(u,v)+\nabla^2u\\
\frac{\partial{v}}{\partial{t}} & = & g(u,v)+\delta\nabla^2v
\end{eqnarray*}
\\
with the the functions f(u,v) and g(u,v) given by:

\begin{eqnarray*}
f(u,v) & = & (u-\frac{u^3}{3}-v)\\
g(u,v) & = & \epsilon(u-\gamma_1v-\gamma_2)
\end{eqnarray*}

Clearly, Barkley took $\gamma_1$=1 and $\gamma_2$=0 in g(u,v), let 
$\delta$=0,  and simplified the cubic equation in f(u,v) by factorising it 
in the model. Now, let us assume that there is no diffusion present, i.e. 
$\nabla^2u$=0. This now changes the system from being a PDE to a ODE. 
Therefore, these simplifications allow us to see what the general dynamics 
are of the model bu using ODE techniques to form a phase portrait diagram. 
The analysis is now given in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Gerneral Dynamics of Barkleys Model}

The nullclines of the system are given by setting $\frac{\partial{u}}{\partial{t}}=0$ and $\frac{\partial{v}}{\partial{t}}=0$. This gives us the following nullclines:

\[\begin{array}{llll}
u=0 & u=1 & u=\frac{v+b}{a} & (\mbox{Fast Nullclines})\\
&&u=v & (\mbox{Slow Nullclines})
\end{array}\]

Whether a nullcline is fast or slow can be determined using singular 
perturbation theory.

Next, we find the steady states of the system, determined by $\frac{\partial{u}}{\partial{t}}=\frac{\partial{v}}{\partial{t}}=0$. This gives us:

\[\begin{array}{lll}
SS_1=(0,0) , & SS_2=(1,1) , & SS_3=(\frac{b}{a-1},\frac{b}{a-1})
\end{array}\]

Now, we must determine whether the steady states of the system are stable or 
unstable. Firstly, the Jacobian of the system is given by:

\[J(u,v)=\left[\frac{\partial{\bf{f}}}{\partial{\bf{u}}}\right],\ 
\mbox{for}\ {\bf{u}}=(u,v),\ {\bf{f}}=(f({\bf{u}}), g({\bf{u}}))\]
\[J(u,v)=\left(\begin{array}{cc}
-3u^2+2u(1+\theta)-\theta & \frac{u^2}{a}-\frac{u}{a}\\
1 & -1
\end{array}\right)\]
\\
where $\theta=\frac{v+b}{a}$. To determine the stability of the system at a 
particular point, we must solve the eigenvalue problem of the system at that 
point . Note that the Jacobian is commonly referred to the Stability Matrix 
(and in Population Dynamics, it is called the Community Matrix). At $SS_1$:

\[J(0,0)=\left(\begin{array}{cc}
-\frac{b}{a} & 0\\
1 & -1
\end{array}\right)\]

Clearly the eigenvalues at $SS_1$ are $\lambda_1=-\frac{b}{a}$ and $\lambda_2=-1$. Hence we can conclude that as long as $a$ and $b$ are both positive or negative, the eigenvalues are both negative, hence $SS_1$ is a 
stable node.

At $SS_2$, the Jacobian is now given by:

\[J(1,1)=\left(\begin{array}{cc}
\frac{1+b-a}{a} & 0\\
1 & -1
\end{array}\right)\]

giving the eigenvalues to be $\lambda_1=\frac{1+b-a}{a}$ and $\lambda_2=-1$. Therefore, the stability of $SS_2$ all depends on the sign of $\lambda_1$. If $\lambda_1$ is negative we get a stable node; if it is positive, $SS_2$ 
will be a sadle point because there will be a negative eigenvalue and a positive eigenvalue. We will look at this closer in the analysis that follows.

Finally, the Jacobian at $SS_3$ is:

\[J\left(\frac{b}{a-1},\frac{b}{a-1}\right)=\left(\begin{array}{cc}
\frac{b(a-b-1)}{(a-1)^2} & -\frac{b(a-b-1)}{a(a-1)^2}\\
1 & -1
\end{array}\right)\]

Now, let us have a look at the phase portrait as it stands:

\begin{figure}[h]
\begin{center}
\begin{minipage}[b]{0.75\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/diagram1.eps}
\caption{Basic Phase Portrait. A typical trajectory is shown by the broken 
line, together with 2 regions shown as S1 and S2. These regions are the 
triangles surrounding these labels.}
\label{BFP}
\end{minipage}
\end{center}
\end{figure}

Let us know determine the conditions for when the model is in an excited 
state.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Excitability for when a$<$1}

As you can see, we have assumed that the gradient of the nullcline given by 
v=au+b (fast nullcline) is smaller than the gradient of the slow nullcline 
given by v=u, i.e. a$<$1. Let us look closer at the mathematics of the 
system for when a$<$1.

Clearly if a$<$1 then there is an intersection of the fast and slow 
nullclines as shown in the diagram above. This means that $\frac{b}{a-1}<0$. 
Now if a$<$1, then b$>$0.

Let us now consider a travelling wave generated by this system:

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/wave.eps}
\caption{A travelling wave in the 'u' field. The wave in the 'v' field will 
generate a similar diagram.}
\label{wave2}
\end{minipage}
\end{center}
\end{figure}

This wave can only be generated if the system is excited. If the speed of 
the wave is $C(\lambda)$, then for the wave to move in a positive direction 
we require:

\[\begin{array}{crcl}
&S_+ & > & S_-\\
\Rightarrow & u & < & \frac{1}{2}\\
\Rightarrow & \frac{v+b}{a} & < & \frac{1}{2}\\
\Rightarrow & b & < & \frac{a}{2} \indent \mbox{at v=0}
\end{array}\]

Consider now $SS_2$. For $SS_2$ to be stable, we require:

\begin{eqnarray*}
\frac{1+b-a}{a} & < & 0\\
\Rightarrow  1+b & < & a
\end{eqnarray*}

This implies that if a$<$1 then b$<$0, which contradicts what we stated 
earlier. Therefore we must have that $SS_2$ is unstable and that:

\[\begin{array}{crcl}
&\frac{1+b-a}{a} & > & 0\\
\Rightarrow & a & < & b+1
\end{array}\]

Hence, for a$<$1, we have:

\[\begin{array}{ccccc}
0 & < & a & < & 1\\
0 & < & b & < & \frac{a}{2}
\end{array}\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Excitability for when a$>$1}

Now let a$>$1. The basic Phase Portrait now looks like:\\
\begin{figure}[h]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/diagram2.eps}
\caption{Basic Phase Portrait for when a$<$1}
\label{BPPsmalla}
\end{minipage}
\end{center}
\end{figure}

Again, a$>$0 and b$>$0, hence $SS_1$ is a stable node.  We know that for 
$SS_2$ to be stable, we require that $\frac{1+b-a}{a}<0$ and for $SS_2$ to 
be unstable, $\frac{1+b-a}{a}>0$. Let us assume that $SS_2$ is unstable:

\[\begin{array}{ccccc}
&\frac{1+b-a}{a} & > & 0\\
\Rightarrow & 1+b-a & > & 0 & \mbox{since a}>0\\
\Rightarrow & b & > & a-1\\
\end{array}\]

Since we also have that b$<\frac{a}{2}$, then b is bounded by 2 lines:

\[a-1<b<\frac{a}{2}\]
Consider now the intersection of these two lines. This intersection will 
represent the maximum values of a and b in which the system is excited:

\[\left\{\begin{array}{ccc}
b & = & a-1\\
b & = & \frac{a}{2}
\end{array}\right.\]
\[\begin{array}{cccc}
\Rightarrow & a-1 & = & \frac{a}{2}\\
\Rightarrow & a & = & 2\\
\Rightarrow & b & = & 1
\end{array}\]

Therefore, for b to be between these 2 lines, we require the following:

\[\begin{array}{ccccc}
1 & < & a & < & 2\\
a-1 & < & b & < & \frac{a}{2}
\end{array}\]

What if $SS_2$ is a stable node? If this is the case, then this would mean 
that $\frac{1+b-a}{a}<0$, hence:

\[\begin{array}{ccccc}
&\frac{1+b-a}{a} & < & 0\\
\Rightarrow & 1+b-a & < & 0 & \mbox{since a}>0\\
\Rightarrow & b & < & a-1\\
\Rightarrow & \frac{b}{a-1} & < & 1
\end{array}\]

Thus, we can therefore say that if $SS_2$ is stable, then $SS_3$ lies between $SS_1$ and $SS_2$ since the coordinates of $SS_3$ are $\left(\frac{b}{a-1},\frac{b}{a-1}\right)$ and as shown above $\frac{b}{a-1}<1$. The Phase Portrait now looks as follows:

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/diagram3.eps}
\caption{Basic Phase Portrait with $SS_3$ between $SS_1$ and $SS_3$}
\label{BPPbetween}
\end{minipage}
\end{center}
\end{figure}

We now need to determine the stability of $SS_3$. Recall from section 2.1.1 
that the stability matrix of $SS_3$ is given by:

\[J\left(\frac{b}{a-1},\frac{b}{a-1}\right)=\left(\begin{array}{cc}
\displaystyle{\frac{b(a-b-1)}{(a-1)^2}} & 
\displaystyle{-\frac{b(a-b-1)}{a(a-1)^2}}\\\\\vspace{-0.3cm}\\
\displaystyle{1} & \displaystyle{-1}
\end{array}\right)\]
\[J\left(\frac{b}{a-1},\frac{b}{a-1}\right)=\left(\begin{array}{cc}
\displaystyle{A} & \displaystyle{-\frac{A}{a}}\\\\\vspace{-0.8cm}\\
\displaystyle{1} & \displaystyle{-1}
\end{array}\right)\]

where A=$\frac{b(a-b-1)}{(a-1)^2}$. Now the eigenvalues of this system are given by the solution to the following eigenvalue problem:

\[\begin{array}{cccc}
& \mbox{DET}(J|_{SS_3}-\lambda I) & = & 0\\
\Rightarrow & \left|\begin{array}{cc}A-\lambda & 
-\frac{A}{a}\\1&-1-\lambda\end{array}\right| & = & 0\\
\Rightarrow & (\lambda-A)(\lambda+1)+\frac{A}{a} & = & 0\\
\Rightarrow & \lambda^2+\lambda(1-A)+\frac{A}{a} & = & 0
\end{array}\]

Therefore, solution to this quadratic equation is:

\[\lambda = \frac{A-1}{2}\pm\frac{\sqrt{(A+1)^2-\frac{4A}{a}}}{2}\]

Now after some algebra, A can be rewritten as:

\[A=\frac{b}{a-1}\left(1-\frac{b}{a-1}\right)\]

Therefore, we now get:

\[\begin{array}{cccccc}
& 0 & < & \frac{b}{a-1} & < & 1\\
\Rightarrow & 0 & < & 1-\frac{b}{a-1} & < & 1\\
\Rightarrow & 0 & < & (\frac{b}{a-1})(1-\frac{b}{a-1}) & < & 1\\
\Rightarrow & 0 & < & A & < & 1
\end{array}\]

Using the above inequality we can see that if we write the eigenvalues as  $\lambda_{\pm}=\frac{\alpha\pm\sqrt{\beta}}{2}$ with $\alpha=A-1$ and $\beta=(A+1)^2-\frac{4A}{a}$ then:

\[\begin{array}{cccccc}
& -1 & < & A-1 & < & 0\\
\Rightarrow & -1 & < & \alpha & < & 0
\end{array}\]

Let us look closer at $\beta$:

\[\begin{array}{cccccc}
& 0 & < & A & < & 1\\
\Rightarrow & 1 & < & A+1 & < & 2\\
\Rightarrow & 1 & < & (A+1)^2 & < & 4\\
\mbox{also} & -\frac{4}{a} & < & -\frac{4A}{a} & < & 0\\
\Rightarrow & 1-\frac{4}{a} & < & (A+1)^2-\frac{4A}{a} & < & 4\\
\Rightarrow & 1-\frac{4}{a} & < & \beta & < & 4
\end{array}\]

We can therefore conclude that if $\frac{1}{4}<\beta<4$ then we have a 
saddle point (we will have a positive and a negative eigenvalue in this 
case); if $0<\beta<\frac{1}{4}$ and $\alpha^2>\beta$ we get a stable node; 
if $0<\beta<\frac{1}{4}$ and $\alpha^2<\beta$ we get a saddle point; and if 
$\beta<0$ we have a stable spiral point, since the eigenvalues will be 
complex with the real part ($\alpha$) being negative.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Excitability for when a=1}

When a=1, we have that the fast nullcline, given by $v=au-b$, and the slow 
nullcline, $u=v$, are parallel. This mean that unless b=0, the 2 nullclines 
will never meet and therefore there will only ever be 2 steady states, 
$SS_1$ and $SS_2$. We shall consider the stability of these states in the 
paragraphs below. If however b=0, we get that every single point on the line 
v=u is a steady state and so we have that the system now has an infinite 
amount of steady state solutions.

Consider now the case when b$\ne$0. $SS_1$ is stable if b$>$0, since a$>$0. 
The stability of $SS_2$ depends on the sign of the first eigenvalue:

\[\begin{array}{ccccc}
&\lambda_1 & = &  \frac{1+b-a}{a} &\\
\Rightarrow & \lambda_1 & = & b & \mbox{since a}=1\\
\Rightarrow & \lambda_1 & > & 0 & \mbox{if b}>0\\
\mbox{and}& \lambda_1 & < & 0 & \mbox{if b}<0
\end{array}\]

So, $SS_2$ is stable if and only if b$<$0, and unstable if and only if 
b$>$0. If $SS_2$ is stable then excitation cannot occur, since no wave 
propagation can occur with the system having 2 stable steady states and no 
unstable steady state. Therefore, $SS_2$ must be unstable and b$>$0.

By a similar argument to that in section 2.1.2 above regarding the direction 
of the propagating wave, we get that $b<\frac{a}{2} \Rightarrow 
b<\frac{1}{2}$. Hence when a=1, 0$<$b$<\frac{1}{2}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Summary}

In summary to this section, we have that for the model to be excited, and 
hence generate waves, the following conditions must be satisfied:
\[\begin{array}{ccccc}
0 & < & a & < & 2\\
a-1 & < & b & < & \frac{a}{2}\\
\mbox{for} && b & > & 0
\end{array}\]

\subsection{A simple test to numerally solve Barkley's model}
Using just the the three Euler methods described above, we conducted a series of simple tests. A C-code was constructed which solved Barkley's model numerically, and produced a data file containing the values of $(u_t,v_t)$ for each t. The number of steps taken was 50,000 and the time-step was varied in each method. The data file was then used, together with Gnuplot, to see what the trajectory looked like. Several of our results are included below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Spiral Waves}
\label{sec:SW}

We will now use the the basic phase portrait developed in Section \ref{sec:BM} to introduce the concept of a spiral wave.
Firstly, we need to draw the action potentials for both the $u$-field and the $v$-field. These are as shown in fig \ref{fig:uv}. Note that the horizontal axis is labelled as $x-ct$ due to the fact that both $u$ and $v$ are wave solutions and are therefore dependent on both space and time. Hence, both $u$ and $v$ can be written as $u=u(x-ct)$ \& $v=v(x-ct)$, where c is the speed of the wave. 

Now, we want to translate this information onto a 2-D plane, since we are looking at spiral waves which are 2-dimensional. So, we take set values of both $u$ and $v$ as shown in figure \ref{fig:uv} and assume that we initially have a broken, plane wave travelling in the positive $x$-direction. In general, the plane wave is finite in the $x$-direction but in the $y$-direction it tends to infinity. A broken wave, i.e. a plane wave that has been "cut-off" at a particular $y$ value, can be generated by a variety of methods, but for spiral waves one method that occurs in cardiac tissue is when a wave of electricity re-enters the tissue and interacts with other waves present, thereby annihilating part of the wave and causing it to be broken.

Hence we get the diagrams as shown in figure \ref{fig:sw}. As we can see, the wave evolves from the diagram on the top left of figure \ref{fig:sw} ending up at the bottom right. The arrows indicate the direction that the $u$-field is moving in. As mentioned above, we consider the evolution of a broken wave travelling initially in the positive $x$-direction. However, due to the interaction of the $v$-field on the $u$-field, the wave starts to move in the $y$-direction as well as the $x-$direction. Eventually, a spiral wave evolves. 

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.22\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/sw1.eps}
\end{minipage}
\begin{minipage}[b]{0.22\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/sw2.eps}
\end{minipage}
\begin{minipage}[b]{0.22\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/sw3.eps}
\end{minipage}
\begin{minipage}[b]{0.22\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/sw4.eps}
\end{minipage}
\caption{Evolution of a Spiral Wave, with the wave evolving from left to right. The $u$-field is denoted by the solid isoline, and the $v$-field is shown as the dotted isoline. The arrows show the directions in which a particular part of the $u$-field is moving.}
\label{fig:sw}
\end{center}
\end{figure}

\subsection{Spiral Wave Tip}
\label{sec:SWT}

To find the location of the tip of the spiral wave is of vital importance. In order to observe and classify the type of motion of the spiral wave, we must locate its tip. There are 2 definitions that are used.

The first definition is that we fix values of $u$ and $v$, i.e. $u=u_*$ and $v=v_*$. This definition was actually used in sections \ref{sec:BM} and \ref{sec:SW} when we introduced the concept of the spiral wave. The 2 isolines bounding the red area ($u$-field) and the blue area ($v$-field) are the values of $u=u_*$ and $v=v_*$ respectively. Their intersection represents the tip of the spiral wave. It must be noted at this point that the values of $u_*$ and $v_*$ must be chosen sensibly. In particular, we also note that the systems we study are excitable systems and therefore $0\le (u,v) <1$. Hence, we must also have $0\le (u_*,v_*) <1$. When FitzHugh introduced his system of PDE's in 1961 \cite{FHN1}, he produced a phase portrait similar to the one we produced in figure \ref{fig:phase}, on which he indicated a region known as \emph{No Man's Land}. This is the region in which the tip of the spiral must be located.

The second definition considers only the $u$-field and sees how it evolves in time. To do this we fix a value of $u$ and let the rate of change of $u$ be zero, i.e. $u=u_*$ and $\frac{\partial{u}}{\partial{t}}=0$.

In our studies, we use the second definition with $u=\frac{1}{2}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Spiral Wave Motion and Dynamics}

\subsubsection{Rigid Rotation}
\label{sec:RW}

\emph{Rigidly Rotating Spiral Waves} (RW's) occur in a periodic system. It has been observed in many numerical studies that the transition from plane wave solutions to RW solution is via a \emph{Hopf Bifurcation}. This Hopf Bifurcation has the affect of introducing a frequency into the system, which we generally call $\omega_1$. The presence of this frequency means that we have periodic solutions present and hence the tip of the spiral wave traces out a circle as shown in figure \ref{fig:rw}. Note that the point of rotation of the RW is fixed.

\begin{figure}[p]
\begin{center}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/rw1.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/rw2.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/rw3.eps}
\end{minipage}
\caption{A rigidly rotating wave ($a$=1.0, $b$=0.25, $\epsilon$=0.01)}
\label{fig:rw}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Meandering Waves}
\label{sec:MRW}

\emph{Meandering waves}, also known as \emph{Modulated Rotating Waves} (MRW's) or \emph{compound waves}, occur in a 2-frequency, quasiperiodic system. The buzzword here is \emph{quasiperiodic}. The 2 frequncies must not be rationally related otherwise we get a phenominon known as \emph{frequency locking}, which does not occur in an excitable system such as what we find in cardiac tissue.

We now have 2 frequencies present, $\omega_1$ and $\omega_2$, with $\omega_1$ being the same frequency as we find in RW's. So, how is this second frequency introduced. It has been observed in many numerical experiments on models that produce spiral wave solution that the transition from RW to MRW is via a Secondary Hopf Bifurcation (also known as \emph{Neimark-Sacker} bifurcation \cite{kuznetsov}). However, it was not until 1990 that Barkley showed that there was numerical evidence that this transition was via a Supercritical Hopf Bifurcation (technically, this is a Supercritical Secondary Hopf Bifurcation) \cite{Bark90}. Hence, this bifurcation has the affect of introducing a further frequency into the system.

So, what we get are spiral waves that trace out "flower" type patterns, with either inward facing petals or outward facing petals. As with RW's, we have that the point of rotation is fixed. Also, the primary frequency, $\omega_1$, determines the motion about the fixed point, whilst the secondary frequency, $\omega_2$, determines the motion of the petals. Also, whether a MRW has inward or outward facing petals all depends on the values of the frequencies. An example of each is shown in figures \ref{fig:mrwout} and \ref{fig:mrwin}.

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwout1.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwout2.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwout3.eps}
\end{minipage}
\caption{MRW's with outward petals ($a$=1.0, $b$=0.2, $\epsilon$=0.01).}
\label{fig:mrwout}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwin1.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwin2.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{chapter2/Spiral_waves/pics/mrwin3.eps}
\end{minipage}
\caption{MRW's with inward petals ($a$=1.0, $b$=0.22, $\epsilon$=0.01).}
\label{fig:mrwin}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transition from periodic to quasiperiodic}

Barkley first introduced his model in a paper published jointly with Mark Kness and Laurette Tuckerman in Physical Review A (1990) \cite{Bark90}. In this paper they indicate that instabilities shown by spiral waves are of much interest. Under certain conditions, the spiral wave rotates with a periodic motion. This wave is then said to be Rotating (RW as described by this report) or simple rotation, as some authors like to call it. However, upon a certain change in the parameters in the system, a second frequency appears and the system becomes quaisperiodic, showing Modulated waves (MRW in this report), or compound rotation. The question of interest is how is this second frequency produced.

It has been known for some time that a Hopf Bifurcation is responsible for the transition from periodic to quasiperiodic motion. This was shown numerically by Lugosi \cite{Lugo89} and also by Skinner et al \cite{Skin89}. They both suggested that the bifurcation looked as if it was supercritical but it was Barkley et al in their 1990 paper who proved that this was actually the case.

They firstly introduce the model, together with the following algorithm to to obtain efficient time stepping in the absence of diffusion:

\begin{eqnarray*}
\mbox{if}\ u^n < \delta, \mbox{then} & &\\
u^{n+1} & = & 0,\\
v^{n+1} & = & (1-\Delta t)v^n,\\
\mbox{otherwise}, & &\\
u_{th} & = & (v^n+b)/a,\\
v^{n+1} & = & v^n+(\Delta/\epsilon)u^n(1-u^n)(u^n-u_{th})
\end{eqnarray*}
\\
where $\delta$ is the thickness of a boundary layer as shown in the following diagram (note that $\delta$ is taken to be small, but Barkley et al do not specify what "small" means in this context).

They then introduce a formula for computing the time stepping of the model \emph{with} diffusion, and this formula is as follows:

\begin{eqnarray*}
6h^2\nabla^2u_{ij} & = & \sum_{r,s}{A_{rs}u_{i+r,j+s}}-20u_{ij}
\end{eqnarray*}

The above formula is the 9-point Laplacian formula using finite differences for $\delta^2u_{ij}$ (as discussed in section 3.1 above), and a similar formula for $\delta^2v_{ij}$ is generated. Taking $u_{ij}$ to be the value of $u$ at the point (i,j), then $A_{rs}$ = 4 for its the point's nearest 4 neighbours, $A_{rs}$ = 1 for the 4 diagonal neighbours and $A_{rs}$=0 otherwise.

These are then used in their numerical experiments to obtain Spiral Wave solutions. Now, the definition of the tip of spiral is given, in Barkley's experiments, as being the intersection of 2 contours, u=1/2 and f(u=1/2,v), implying that v=(a-2b)/2. He has chosen this definition as it is least sensitive to spatial discretisation as u=1/2 is directly in the centre of the range of the u field. Therefore, any error occuring in the numerical calculations will be minimisied.

Now, in order to provide evidence of the presence of a supercritical Hopf bifurcation, Barkley et al computed the decay rates to simple rotations on one side of the bifurcation and on the other side, they computed the ratio of the amplitudes of the compound waves formed. Remember from the definitions section that MRW's (compound waves) have 2 frequencies and are constructed by taking 2 circles - the primary circle with radius r$_1$ and secondary circle with r$_2$ - and, with the tip of the spiral located at a fixed point on the secondary circle, a flower pattern is traced out when the primary and secondary circles rotate with frequencies $\omega_1 \ \mbox{and} \ \omega_2$ respectively. The amplitudes of the compound waves are simply the radii of these circles. In reality, we find that the secondary circle is in fact an ellipse but is "almost" circular. Therefore, the radius r$_2$ is actually the maximum value of the radius.

Barkley et al then ploted the ratio of the secondary radius to the primary radius (r$_1$/r$_2$) against the parameter $a$, and also on the same plot, the decay rate, $\lambda$, against $a$, therefore generating the following plot:

As can be seen, the amplitude of the secondary mode grows from zero at the same point, $a_c$, where the decay rate goes through zero. It can also be seen that near the bifurcation point, the growth of the secondary radius is given by a power law $\sim \frac{1}{2}$.

Hence, these observation provide the first conclusive evidence that the transition from simple to compound rotation is via a supercritical Hopf Bifurcation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Spiral Wave Dynamics}
In 1994, 2 very similar papers were published - the first by Dwight Barkley in Physical Review Letters (PRL) \cite{Bark94a} and the other by Dwight Barkley and Ioannis Kevrekidis in Chaos \cite{Bark94b}. The first of these papers was rather short due to it appearing in PRL, and therefore a lot of the analysis was left out. The second paper provided further details of the analysis work done, therefore filling in various gaps in the first paper, together with an overview of the different types of motion of Spiral Waves. In this section, we will give brief reviews of these papers and provide further analysis that we feel is relevant in the understanding of the concepts introduced in these papers.

In the PRL paper, Barkley firstly mentions that Spiral Waves exhibit different types and that these motions are all dependent on the the values of the parameters used. This is demonstrated by Barkley in the parametric portrait shown below: 

\begin{figure}[htbp]
\begin{center}
\begin{minipage}{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/Bark.eps}
\caption{A Parametric Portrait with $\epsilon = 0.02$}
\label{BarkPara}
\end{minipage}
\end{center}
\end{figure}

As can be seen, there are different regions representing the various motions of the Spiral Waves: $N$ represents regions of no waves; $MRW$ are of course Modulated Rotating Waves; $MTW$ are Modulated Travelling Waves (Drifting Waves); and $RW$ represents Rotating Waves.

Of particular interest to us are MRW's. Their motion is quasiperiodic, which is seen as periodic from a rotating frame of reference. As mentioned in section 4.2, the transition from RW to MRW occurs via a Supercritical Hopf Bifurcation, in which an additional frequency, $\omega_2$, is introduced. When our frame of reference is taken as rotating with frequency equal to that of the primary frequency, $\omega_1$, we find that the because there is now only one frequency relative to this rotating frame of reference, then the MRW appears to rotate so as the tip traces out a circle, as in RW.

Now, the boundary between RW's and MRW's is known as the Hopf Locus. Within this boundary is another boundary (locus) which separates MRW's with inward petals from those with outward petals. Along this locus MTW's can be found. The intersection of these loci is call the \emph{"Codim-2 Point"}, or \emph{"The Orgainising Centre"}. Very close to this point are areas of RW's, MRW's with both inward and outward pointing petals, and also MTW's. Therefore, understanding the dynamics of this point is critical in understanding the dynamics of the transition from RW to MRW.\\


\subsection{EZSpiral and Numerical Methods}
As mentioned in the Introduction, Barkley devised a program that graphically 
depicted what Spiral Waves were produced under a particular set of 
conditions and parameters, and how these waves evolve in time. This program 
is called EZSpiral and is available for download from Barkley's 
webpage \cite{barkweb}.

Barkley's program is written in C code with a free licence so that it can be ammended for the users usage. Once made using the usual MAKE command, the program is ready to use. As well as the C codes and header files, there is also a file called \emph{task.dat}, which contains the numerical and physical parameters needed to run the program. These parameters can be changed accordingly by ammending the \emph{task.dat} file. The parameters used in our experiments are described in Chappter 5. A variety of numerical techniques are implemented in EZSpiral in order to ensure that the solutions produced are as accurate as possible. These methods are now described below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Numerical Methods used in EZSpiral}

Let us now look at the numerical methods that are incorporated into EZSpiral. There are 4 main methods that are used, viz Explicit Forward Euler Method, Semi-Implicit Forward Euler Method, the 9-point Finite-Difference Laplacian Method and the 5-point Finite-Difference Laplacian Method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Explicit Forward Euler Method}

Firstly, let us consider Barkley's model without any diffusion. This gives us the following system:

\begin{eqnarray*}
\frac{\partial{u}}{\partial{t}} & = & f(u,v)\\
\frac{\partial{v}}{\partial{t}} & = & g(u,v)
\end{eqnarray*}

For the time being let us look just at the $u$-field. Let $u_t$ denote the value of $u$ at time $t$ and let $h_t$ denote the time step. Therefore, we can rewrite the equation for the $u$-field above as follows:

\begin{eqnarray*}
\frac{u_{t+h}-u_t}{h_t} & = & f(u_t,v_t)\\
\Rightarrow \frac{u_{t+h}-u_t}{h_t} & = & \frac{1}{\epsilon}u_t(1-u_t)(u_t-u_{th})\\
\Rightarrow u_{t+h} & = & u_t+h_t\frac{1}{\epsilon}u_t(1-u_t)(u_t-u_{th})
\end{eqnarray*}

Similarly, an equation for $v_{t+h}$ can also be found:

\begin{eqnarray*}
v_{t+h} & = & v_t+h_t(u_t-v_t)
\end{eqnarray*}

Given a suitable, small time-step, $h_t$, together with appropriate initial conditions, we can use this method to numerically calculate the values of $u_t$ \& $v_t$ for a set amount of steps.

This method, i.e. arranging the original PDE's into the above form, is known as the Explicit Forward Euler Method. Barkley, in applying this method to his model without diffusion, found it to be accurate in the fast regions as long as $h_t \approx \epsilon$ is the maximum time step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Implicit Forward Euler Method}

This particular method is very much similar to the Implicit method. However, instead of using the form:

\begin{eqnarray*}
\frac{u_{t+h}-u_t}{h_t} & = & f(u_t,v_t)
\end{eqnarray*}

we now use:

\begin{eqnarray*}
\frac{u_{t+h}-u_t}{h_t} & = & f(u_{t+h},v_{t+h})
\end{eqnarray*}

This now gives us equations for $u_t$ \& $v_t$ in terms of $u_{t+h}$ \& $v_{t+h}$ and hence enables us to work backwards from a given set of values to the initial values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Semi-Implicit Forward Euler Method}

If we wish to take a large time-step then we need to use the Semi-Implicit form of the Euler method. In this instance, we use a mixture of both the implicit method and the explicit method as follows:

\begin{eqnarray*}
\frac{u_{t+h}-u_t}{h_t} & = & f(u_t,u_{t+h},u_{th})\\
\Rightarrow u_{t+h} & = & u_t + \frac{h_t}{\epsilon}u_{t+h}(1-u_t)(u_t-u_{th})\\
\mbox{if} \ u_t & \leqslant & u_{th}\\
\mbox{and} \ u_{t+h} & = & u_t + \frac{h_t}{\epsilon}u_t(1-u_{t+h})(u_t-u_{th})\\
\mbox{if} \ u_t & > & u_{th}
\end{eqnarray*}

The conditions detailed underneath the above expressions for $u$ are clear to understand if we consider the rearrangement of the above as detailed below. We consider the above using $u_{t+h}=F(u_t,u_{th})$:

\begin{eqnarray*}
F(u_t,u_{th}) & = & \frac{u_t}{1-\frac{h_t}{\epsilon}(1-u_t)(u_t-u_{th})}\\
\mbox{if} \ u_t & \leqslant & u_{th}\\
\mbox{and} \ F(u_t,u_{th}) & = & \frac{u_t+\frac{h_t}{\epsilon}u_t(u_t-u_{th})}{1+\frac{h_t}{\epsilon}u_t(u_t-u_{th})}\\
\mbox{if} \ u_t & > & u_{th}
\end{eqnarray*}

Now, $u_{t+h} > 1$ for all t in Barkley's model for waves to be generated. Therefore, it is clear from the first equation above that $\frac{h_t}{\epsilon}(1-u_{t+h})(u_t-u_t)<0$ to guarantee that $u_{t+h}$ is to be positive. Now, as mentioned earlier we use the Semi-Implicit method if we want a larger time-step, in particular we use this method if $h_t > \epsilon \ \Rightarrow \ \frac{h_t}{\epsilon}>1 $. Hence, since $(1-u_t)>0$ then we must have that $(u_t-u_{th}) \leqslant 0 \ \Rightarrow \ u_t \leqslant u_{th}$.

A similar argument is used to show the second condition. Again, we require $u_{t+h}>0$. This therefore means that we the denominator is positive. Hence, to guarantee this condition, we need that $\frac{h_t}{\epsilon}u_t(u_t-u_{th})>0$. Now, $\frac{h_t}{\epsilon}>0$ and $u_t>0$ hence $u_t-u_{th}>0 \ \Rightarrow \ u_t>u_{th}$.

To sumerise for the Euler Methods, we can see that for small $\frac{h_t}{\epsilon}$, we use the Explicit Method (note that the Explicit method can be derived from the expressions for the Semi-Implicit method by expanding the denominators in the expressions for $F(u_t,u_{th})$ above). For large $\frac{h_t}{\epsilon}$, we need to use a Semi-Implicit Methed and find that we can simplify the expressions for $F(u_t,u_{th})$ as follows:

\[\begin{array}{rclc}
F(u_t,u_{th}) & = & 0 & \mbox{if} \ u_t < u_{th}\\
& = & u_{th} & \mbox{if} \ u_t  = u_{th}\\
& = & 1 & \mbox{if} \ u_t  > u_{th}
\end{array}\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Five-Point Finite-Difference Laplacian Method}

The Forward Euler Methods as described above efficiently solve the system, numerically, in the absense of diffusion. Therefore, we now need to introduce a scheme which looks after the diffusion term.

Firstly, let us take the Laplcian in just one dimension and consider the following diagram:

\begin{figure}[htbp]
\begin{center}
\psfrag{A}[tl]{$u$}
\psfrag{B}[tl]{$\frac{\partial{u}}{\partial{x}}$}
\psfrag{C}[tl]{$\frac{\partial^2{u}}{\partial{x^2}}$}
\psfrag{D}[tl]{$u_n$}
\psfrag{E}[tl]{$u''_n$}
\psfrag{F}[tl]{$u_{n-1}$}
\psfrag{G}[tl]{$u_{n+1}$}
\psfrag{H}[tl]{$u'_{n-\frac{1}{2}}$}
\psfrag{J}[tl]{$u'_{n+\frac{1}{2}}$}
\includegraphics[width=0.65\textwidth]{chapter2/Spiral_waves/pics/laplacian}
\end{center}
\caption{Numerical dynamics of the Laplacian}
\label{fig:laplacian}
\end{figure}

Using the argument for the Explicit Forward Euler Method, we can see that:

\begin{eqnarray*}
u'_{n-\frac{1}{2}} & = & \frac{u_n - u_{n-1}}{h_x}\\
u'_{n+\frac{1}{2}} & = & \frac{u_{n+1} - u_n}{h_x}
\end{eqnarray*}

Similarly, we can get an expression for the second derivative at the nth stage:

\begin{eqnarray*}
u''_n & = & \frac{u'_{n-\frac{1}{2}} - u'_{n+\frac{1}{2}}}{h_x}\\
\Rightarrow u''_n & = & \frac{u_{n-1}-2u_n+u_{n+1}}{h_x^2}
\end{eqnarray*}

This is the Numerical Simulation of the Laplacian in one dimension. Let us now consider the Laplacian in 2 dimensions, where $u$ is differentiated with respect to both $x$ and $y$. In the above one dimension case, we could assume that this was in 2 dimensions but keeping $y$ constant. We can perform a similar task but keeping $x$ constant.

Let us rewrite the above equations for the Laplacian as follows:

\begin{eqnarray*}
\frac{\partial^2{u_{n,m}}}{\partial{x^2}} & = & \frac{u_{n-1,m}-2u_{n,m}+u_{n+1,m}}{h_x^2}
\end{eqnarray*}
\\
where $u_{n,m}$ represents the $u$ term at position $(n,m)$. This equation represents the Laplacian when the $y$ term is kept constant and therefore we can similarly represent the Laplacian with the $x$ term constant as follows: 

\begin{eqnarray*}
\frac{\partial^2{u_{n,m}}}{\partial{y^2}} & = & \frac{u_{n,m-1}-2u_{n,m}+u_{n,m+1}}{h_x^2}
\end{eqnarray*}

Combining these equations to represent the complete 2 dimensional Laplacian, we get:

\begin{eqnarray*}
\nabla^2{u_{n,m}} & = & \frac{u_{n-1,m}+u_{n+1,m}+u_{n,m-1}+u_{n,m+1}-4u_{n,m}}{h_x^2}
\end{eqnarray*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Nine-Point Finite-Difference Laplacian Method}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{General notes regarding the implementation of the above methods in EZSpiral}

In order to use the above methods in EZSpiral there are several physical and numerical parameters that we must be aware of and use suitably. These parameters are the size of the grid in which we are carrying out our numerical tests, the number of grid points, and the time step.

Let us denote the length of the grid by $L$ (a "physical" parameter) and the number of grid points ("numerical" parameter) by $N$. In a 2 dimensional grid, we have that the area of the grid is $L^2$ and the total number of points is $N^2$. Now, the spacing between each point is the length of a line in the grid divided by the total number of spaces on that line (if there are $N$ points of the line of length $L$, then there will be a total of $N-1$ spaces between consecutive points). Hence, the "space-step", $h_x$, is given by $h_x=\frac{L}{N-1}$.

Now, for practical purposes, we want to keep the time step, $h_t$ constant throughout a run of calculations. Therefore, we set $h_t=\frac{L^2}{5(N-1)^2}$. The choice of the numerical constant in the denominator (in our case 5), is arbitrary and can be adjusted to suit particular needs. For EZSpiral, this choice of constant was found to produce meaningful results.

As we will see in Chapter 5, the choice of $L,\ N$ becomes important with certain choices of the physical parameters $a,\ b, \ \epsilon$, and this will be explained in detail in Chapter 5.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Numerical Analysis on Barkley's Model}

In this chapter, we describe numerical work that we undertook on Barkley's 
Model. Barkley undertook a similar analysis and used the value of 
$\epsilon$=0.02. Barkley then produced a parametric portrait and this is 
shown in his 1994 paper \cite{Bark94a}. This parametric portrait clearly shows the 
boundaries between regions of No Waves (NW), Rotating Waves (RW's) and 
Modulated Rotating Waves (MRW's), otherwise known as meandering waves. 
Within the region of MRW's we have inward and outward petals together with a 
locus along which there are Modulated Travelling Waves.

In our analysis, we use $\epsilon$=0.01. The results, as will be seen, shown 
several interesting results. Firstly, we describe how the numerical analysis 
was carried out, what tools were used and any modifications that were made. 
Then, we will produce our results ending with a concludion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Methods}

We used EZSpiral throughout this exercise to produce the data required to 
draw the parametric portrait. In order to run EZSpiral, we had to install 
all the necessary C codes and header files onto a UNIX account, and MAKE the 
program as instructed by Barkley. Once the program was running, an X-Window 
would appear which displayed the spiral wave (if it existed), for the 
particular values of parameters $a$ and $b$. The values of $a$ and $b$, 
together with the type of wave produced (if any) were then recorded for 
later analysis. Included with the C codes etc was a file named $task.dat$. 
This contained information about all the parameters and physical properties 
of the space in which the wave was to be generated. For the main results in 
this exercise the only parameters that were varied were $a$ and $b$, with 
the following being kept constant throughout (however, see below for refined 
tests):

$\indent\bullet$ The box length $L_x$ (=$L_y$) was kept at 30.\\
$\indent\bullet$ The number of grid points in each direction $N_x$ (=$N_y$) 
was fixed at 121.\\
$\indent\bullet$ The parameter $\epsilon$ was, of course, equal 0.01 
throughout the exercise.\\
$\indent\bullet$ The number of steps to take was 5,000.\\
$\indent\bullet$ The time step, $h_t$, was kept at 0.0125 and the space 
step, $h_x$, at 0.25.\\
$\indent\bullet$ The maximum time to run the program was 62.5 secs.

Therefore, the space step, $h_x$, and time step, $h_t$, where kept constant 
throughout the first part of the exercise, but as detailed below, we had to 
make changes to these steps in order to verify particular results.

In order to create the set of data, we firstly kept the parameter $a$ 
constant and varied $b$. The first "line" of data we produced for our phase 
diagram, was rather detailed as we needed to establish where the particular 
boundaries between different types of motion where situated. Once the first 
line had been accurately reproduced, we could then change parameter $b$ to 
another fixed value and then vary $a$ with the knowledge that certain 
boundaries existed. This continued until enough data was gathered to produce 
a phase diagram.

However, in order to make sure that the boundaries were as accurate as 
possible, we then repeated the exercise as described in the paragraph above, 
but this time keeping $a$ constant and varying $b$.

During the investigation, we came across some waves for which it was not 
possible to classify their motion from the X-Window generated, due to the 
smallness of the tip path produced. In these cases, we firstly checked the 
tip path using Gnuplot (see below). However, it was still not possible in 
several cases to determine exactly how the wave was behaving. Therefore, we 
refined the tests by varying the parameters of the system as follows:

$\bullet$ Test I - Decrease in $t_s$ (thus decrease in $h_t$) say twice and 
increase the interval between outputs twice.\\
$\bullet$ Test II - Increase $N_x$ at fixed $L_x$, say twice (thus 
decreasing $h_x$ twice and decrease $h_t$ fourfold), and therefore increase 
the interval between outputs fourfold.\\
$\bullet$ Test III - Increase in both $N_x$ and $L_x$, say both twice (thus 
both $h_x$ and $h_t$ remain the same, and the interval between the outputs 
remains the same).\\
$\bullet$ Test IV - Move the initial position of the spiral to one side, say 
by $1/10^{th}$ of the box size.

These tests enabled us to therefore determine exactly what the motion of the 
wave was for a particular set of parameters and hence we were then able to 
produce a phase portrait diagram as shown in the results section below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Results}

As mentioned above, EZSpiral was run using particular parameters. The 
results would then be recorded and the parameters would then be classied as 
NW, RW or MRW. If MRW, then the orientation of the petals would also be 
recorded (i.e inward, outward or MTW).

It was clear from the outset that the diagram was going to have an "extra" 
region, compared with the diagram produced by Barkley [2]. What makes this 
particular region interesting is that it appears outside of the boundary of 
excitablilty. This issue will be discussed in the conclusion that follows. 
The parametric portrait is now produced below but indicting certain regions 
and points, which will be explained further on:

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.8\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/num_portrait_fig2}
\caption{Parametric Portrait of Barkley's Model with $\epsilon$=0.01. The 
region surrounded by a blue boundary is a region of MRW's. Points A - G 
relate to the points that are described in detail in section 2.1. The other 
points shown on the above figure, are the other points that were tested 
during this analysis and classified accordingly.}
\label{paraport}
\end{minipage}
\end{center}
\end{figure}

As you can see from Fig.1, this new region appears to within the RW 
boundary, to the right of the MRW region. In this region are MRW's, but 
instead of having inward petals to the left of the region and outward petal 
to the right, we have outward petals to the left and inward petals to the 
right. We can almost conclude that this region is a diminished reflection of 
the other MRW region. From now on we will refer to the MRW region on the 
left of Fig.1 as MRW(L) and the one on the right as MRW(R).

When we first observed the MRW(R) region, we assumed that there was an error 
with the calculations being produced. Therefore, we ran the four refined 
tests mentioned in the previous section on a point in this region and points 
in the other regions, in order to verify the validity of our results. Also, 
there were certain point in the RW region, between the 2 MRW regions, that 
were behaving in a rather chaotic manner. Hence, several of these points 
were tested too.

Having run the refined tests, we then used Gnuplot to verify our results and 
the graphs produced are shown below. Fig.1 above indicates where about on 
the parametric portrait these points are located.

In the following figures the legend is the same in each of them. The legend 
appears in figure \ref{pointA} and it is then assumed that the reader knows 
what the legend will be in figures 3-13.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{EZSpiral Test Results and Figures}

Ezspiral was used, as previously stated in this report, to determine the 
motion of the wave at particular parametric coordinates. Many coordinates 
were used throughout this exercise (shown as dots on the parametric 
portrait) but we will consider just several of these in the following 
subsection. Note that in all of the following figures, we have plotted each 
test in such a way as to superimpose them as best as possible. This enables 
us to compare the plots for each test more accurately.

Consider firstly the points 'A' and 'B', as shown on the parametric 
portrait. The Gnuplot graph is shown below as figures 2 and 3:

\begin{figure}[htbp]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test241etc.eps}
\caption{Point A for a=0.85 and b=0.2}
\label{pointA}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test244etc.eps}
\caption{Point B for a=0.7 and b=0.1}
\label{pointB}
\end{minipage}
\end{figure}

As one can see for point A in figure \ref{pointA}, the tip path trajectory 
is clearly a circle, and hence the motion of the spiral wave in this 
instance is Rigidly Rotating (RW). All 5 tests (the original plus 4 further 
refined tests) produce the same result, i.e. a RW. As one would expect, when 
all the tip trajectories from the tests are viewed from the same scale, as 
in Fig 2, the radius of the circle traced out is not the same in each case. 
The Orginal Test, together with Tests III and IV, all give approximately the 
same radius. This is expected as the space step, $h_x$, is unaltered in each 
case. In Test I, the time step, $h_t$, is reduced and therefore the radius 
of the circle traced out is accordingly reduced. Finally, in Test II, the 
space step is decreased and hence the radius of the trajectory is also 
decreased.

We can therefore conclude that this particular wave located at point A is 
definitely within a region of RW's.

From figure \ref{pointB} above, it is clear that for point B the wave 
produced is a modulated wave and that the petals are pointing outward. 
Closer inspection of Fig. 3 shows that Tests I and II produce a slightly 
smaller projection and this can be explained with the same arguments as 
above for point A.

The next three figures all come from points taken in the region of RW's 
between the two MRW regions. Some very interesting results arose out of this 
particular region.

Firstly, let us consider points C and D. The graphs of the tip trajectories 
are shown below:

\begin{figure}[htbp]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test247etc.eps}
\label{pointC}
\caption{Point C for a=1.1 and b=0.15}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test250etc.eps}
\label{pointD}
\caption{Point D for a=1.3 and b=0.1}
\end{minipage}
\end{figure}

For point C, the first run of EZSpiral on this particular set of parameter 
was not very conclusive, mainly due to the size of the trajectory produced 
in the X-Window. Further tests on this point, together with the help of 
Gnuplot clearly showed that the wave, after an initial period of moving from 
its center of rotation, settled down to be a RW. This phenomenon was 
observed by Winfree in his 1991 paper \cite{Winf91}. Therefore, it can be concluded 
that the motion of the spiral can be said to be Rigidly Rotating.

For point D, we are now protruding into the region of no excitation, and in 
this region the results start to become interesting. When Ezspiral was first 
run with the above values for $a$ and $b$ as stated in figure 4, producing 
the orginal test, it was not very clear what was happening, due to the 
motion of the tip projecting a very small image in the X-Window. Once the 
program had completed its run, a Gnuplot graph was generated with the 
tip.dat file which showed that the motion of the tip indicated that the wave 
was Rigidly Rotating (RW). However, when the refined tests were run and the 
results plotted with Gnuplot, it transpired that the wave displayed Rigid 
Rotaion for Tests I - III but for Test IV, the wave appeared to be slowly 
Meandering. This seemed to indicate that there was a boundary effect on the 
wave (recall that in test IV, the wave was displaced from it's original 
position, being moved closer to the boundary). A Further test was run, in 
which the number of plots was increased from 5,000 to 20,000 and this seemed 
to conclude that the wave in this case was indeed Rigidly Rotating.

Before moving on to point E, we ask the reader to note the size of the scale 
of the axes in the above figure. If one looks closely at the RW's produced, 
the radius of the circle produced by the RW is approximately 0.12 space 
units (su). The space step of the Original test is approximately 0.25 su's 
and therefore the radius of the trajectory is less than half of the space 
step, i.e. extremely small. We could conclude that the due to the radius 
being so small, the wave is almost stationary and therefore rotation occurs 
about a fixed point.

The next set of parameters plotted raised eyebrows when the following figure 
was produced. Again, this set of parameters are outside of the region of 
excitability:

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test253etc.eps}
\caption{Tests for point E using a=1.4 and b=0.2}
\label{pointE}
\end{minipage}
\end{center}
\end{figure}

From observing what was happening in the X-Window, it appeared that the tip 
was not moving at all, but rotation was occuring about a fixed point. 
Running the usual refined tests and plotting the results using Gnuplot, it 
can be seem that a very odd "spinal" shape is produced. Note also that the 
scale of the axes show that the trajectory of the tip traced out is in a 
very small domain, spanning approximately 0.1 su's.

After careful consideration, we decided to change the position of the Spiral 
Tip by amending the C code for EZSpiral. In the file eztip.c, the tip of the 
spiral wave is defined as the intersection of the 2 contours U\_CONT and 
V\_CONT, given by:

\begin{eqnarray*}
  \mbox{U\_CONT} &=& 0.5 \\
  \mbox{V\_CONT} &=& \frac{a}{2} - b
\end{eqnarray*}

U\_CONT was changed to 0.4 and the EZSpiral was re-made and re-run using the 
orginal set of parameters. After this run, U\_CONT was then changed to 0.6 
and the same process was followed. These 2 further tests showed that the 
wave was indeed Rigidly Rotating for this particular set of parameters. The 
orginal tests with U\_CONT = 0.5, just happened to be where the spiral tip 
was stationary. The diagram of the tip path for the particular values of 
U\_CONT is shown below:

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{1\linewidth}
\centering
\includegraphics[width=0.5\textwidth]{chapter2/Spiral_waves/pics/PointE_UCont.eps}
\caption{Tests conducted on Point E with U\_CONT = 0.4 and U\_CONT = 0.6.}
\label{pointEUC}
\end{minipage}
\end{center}
\end{figure}

Next we take a set of parameters that show a point in the RW region of Fig. 
1, located on the far right hand side between the regions of NW and MRW(R). 
Again this is in the region of no excitability:

\begin{figure}[h]
\begin{center}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test259etc.eps}
\caption{Tests for point F using a=1.7 and b=0.2}
\label{pointF}
\end{minipage}
\end{center}
\end{figure}

As one can see, the wave is clearly Rigidly Rotating and all tests performed 
on this set of parameters point to this conclusion.

The final point was the point that brought about the most discussion in this 
exercise. Consider the following figure:

\begin{figure}[h]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test256etc.eps}
\caption{Point G for a=1.62 and b=0.2}
\label{pointG}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/retest_a162_b02_60000.eps}
\caption{"Snail Shell" effect in point G}
\label{Snail}
\end{minipage}
\end{figure}

The above figure \ref{pointG} shows that there is something not quite right 
about the tests that were conducted. It is clear that this motion does not 
display meandering (MRW) waves as such because the interval between each 
petal varies. In fact, having run this test for 60,000 plots rather than 
5,000, it was clear that a "Snail Shell" shape is generated by the tip, as 
can be seen in the above figure \ref{Snail} on the right hand side (note 
that when the figure was constructed using Gnuplot, only points between the 
50th and 600th were included in order to show the "Snail Shell" shape).

We therefore ran the refined tests again, but this time changing U\!\_CONT 
and V\!\_CONT to 0.4 and with 20,000 plots. The results produced the 
following figures:

\begin{figure}[htbp]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test348etc}
\caption{Point G using U$\_$CONT=0.4}
\label{GUCONT}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/test348apart}
\caption{Point G using U$\_$CONT=0.4 but showing the individual plots}
\label{Apart}
\end{minipage}
\end{figure}

Test I and II clearly show that the spiral is MRW whilst Tests III and IV 
show that the wave, after an initial period of displaying the "Snail Shell" 
affect, is RW. Therefore, we can conclude that the physical parameters set 
in this model for $a=1.62$ and $b=0.2$ are not sufficient. Therefore, we 
decided that we must change these conditions as follows:

\begin{eqnarray*}
  L_x &=& 60 \\
  N_x &=& 484 \\
\mbox{Steps} &=& 120,000
\end{eqnarray*}

The physical affect of these changes is that the box size has inceased in 
each direction by 2; the number of points on each axis has increased by 4; 
therefore the overall change in the space step, $h_x$ has decreased by 2. 
Hence the time step, $h_t$ has increased by 4. For a run of EZSpiral that 
took only a minute to run, it was calculated that the new run would take 
approximately 6.5 hours, at least. Running the tests overnight, we find that 
the following graphs are produced:

\begin{figure}[htbp]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/retest_a162_b02}
\caption{Point G using a more appropriate set of spatial parameter}
\label{Gbetter}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{chapter2/Spiral_waves/pics/retest_a162_b02_apart}
\caption{Point G with better spatial parameters, but with the plots shown 
separately}
\label{Gbetterapart}
\end{minipage}
\end{figure}

Thus, in a larger medium the motion of the spiral is clearly MRW. We can 
therefore conclude that spirals located in this region display meandering 
motion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Conclusion}

This particular analysis of Barkley's model produced some interesting 
results. From Fig.1, we can see that in the region of excitability, we come 
across regions where there is spiral wave activity. Some of these spirals 
rigidly rotate, while other spirals display quasi-periodic motion, i.e. 
meander. It is interesting to note that spiral waves are still being 
generated in a region of no excitability (see section 2 above), for when 
$b<a-1$. This now proposes further questions as to why waves can be 
generated in this region, and this can be the basis for further analysis.

Going back to the parametric portrait in Fig. 1, we note that, compared to 
Barkley's parametric portrait for $\epsilon$=0.02 [2], the region of 
mendering waves is somewhat stretched and larger. This agrees with 
observations by Hakim and Karma in their 1999 paper \cite{Hakim99}.

We conclude that through numerical observations, spiral wave activity is 
present in regions of "non-excitability". This particular may well consist 
of a particular type of excitability but one that is not yet documented.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The ODE Model}
\label{sec:ODE}

Barkley et al (1994) introduced a system of ODE's which, when numerically solved, produced patterns that were similar to the patterns produced by the PDE system, i.e Meandering patterns were observed \cite{Bark94a,Bark94b}. The system takes advantage of 2 particular properties of spiral wave solutions:

\begin{enumerate}
\item 1) Invariance under Euclidean Symmetry; and\\
\item 2) Presence of a Supercritical Hopf Bifurcation.\\
\end{enumerate}

However, the system is \emph{a priori} in the sense that when Barkley et al introduced this system, the Bifurcation Theory at that time was insufficient to justify the production of a set of ODE's from the PDE system. They simply introduced this system, and indicated that it worked by showing an example. The system is as follows:

\begin{eqnarray*}
\dot{p} & = & v \\
\dot{v} & = & v\cdot \{f(|v|^2,w^2)+iw\cdot h(|v|^2,w^2)\}\\
\dot{w} & = & w\cdot g(|v|^2,w^2)
\end{eqnarray*}

As we can see, there are 3 dependent variables. $p$ is the position vector and is complex; $v$ is the velocity vector and is also complex; and $w$ is the frequency and is real. We now let $p=x+iy$ and $v=se^{i\phi}$, where $x,y$ are the position coordinates, $s$ is speed, and $\phi$ is the angle between the x-axis and the line from the origin to the point ($x,y$). We are therefore left with a 5-dimensional system of ODE's:

\begin{center}
$\dot{x}=s\cos(\phi)$, $\dot{y}=s\sin(\phi)$\\
$\dot{\phi}=w\cdot h(s^2,w^2)$, $\dot{s}=s\cdot f(s^2,w^2)$, $\dot{w}=w\cdot g(s^2,w^2)$
\end{center}

As you can see, we have 3 unknown functions, $f(s^2,w^2)$, $g(s^2,w^2)$ and $h(s^2,w^2)$, and it is up to the researcher to define exactly what these functions are. Barkley et al took these functions and expanded them, using Taylor, as follows:

\begin{eqnarray*}
f(s^2,w^2) & = & \alpha_0+\alpha_1s^2+\alpha_2w^2+\alpha_3s^4\\
g(s^2,w^2) & = & \beta_0+\beta_1s^2+\beta_2w^2\\
h(s^2,w^2) & = & \gamma_0
\end{eqnarray*}

After assigning specific values to $\alpha_0$, $\alpha_3$, $\beta_0$, $\beta_1$ and $\beta_2$, and letting $\xi=s^2$ and $\zeta=w^2$, we get the following reduced system:

\begin{eqnarray*}
\dot{\xi} & = & 2\xi f(\xi,\zeta)\\
\dot{\zeta} & = & 2\zeta g(\xi,\zeta)
\end{eqnarray*}

where:

\begin{eqnarray*}
f(\xi,\zeta) & = & -\frac{1}{4}+\alpha_1\xi+\alpha_2\zeta-\xi^2\\
g(\xi,\zeta) & = & \xi-\zeta-1\\
h(\xi,\zeta) & = & \gamma_0
\end{eqnarray*}

We can now take this reduced system and use our usual dynamical system and bifurcation analysis to shown that, for $\alpha_1=\frac{10}{3}$, there is a Hopf Bifurcation at $\alpha_2=-5$ and $\gamma_0=\sqrt{28}$.

In order to verify that the patterns produced by the system of ODE's are the same as those produced by the PDE's, we created a simple C program which numerically solved the 5-dimensional system of ODE's with the parameters $\alpha_1$, $\alpha_2$ and $\gamma_0$ being the parameters that are varied, with the other parameters being kept at the values specified above. We observed that the patterns produced were the same as those produced by the PDE system. One of the patterns is shown in fig \ref{fig:ode}.

\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/tip1.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/tip2.eps}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=0.9\textwidth]{chapter2/Spiral_waves/pics/tip3.eps}
\end{minipage}
\caption{Results from numerical analysis of the ODE system taken from the same tip file but at different time intervals}
\label{fig:ode}
\end{center}
\end{figure}

As we can see, a clear "flower" pattern develops. Furthermore, when we view the pattern at the latter stage, we can see that the trajectory is forming a dense orbit on the 2-Torus, which is then projected onto the 2-D plane.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{chapter2/Spiral_waves/ODEsolve}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{chapter2/Spiral_waves/fit_ODEsolve_data}


==> chapter6/defs.tex <==
\newtheorem{thm}{Theorem}[section]

\theoremstyle{definition}	

\newtheorem{defn}[thm]{Definition}

\newcommand{\ez}{EZ-Freeze }

%%%%%%%%%%%%%%%%% Group Actions etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dd}{\textrm{d}}
\newcommand{\dT}{\textrm{T}(g)}
\newcommand{\ddT}{\textrm{T}(dg)}
\newcommand{\dTddT}{\textrm{T}(g+dg)}
\newcommand{\dTi}{\textrm{T}(g^{-1})}
\newcommand{\ddTi}{\textrm{T}(dg^{-1})}
\newcommand{\ddTcom}{\textrm{T}(\{\textbf{c}dt,\omega dt\})}

%%%%%%%%%%%%%%%%% Bold letters and Symbols %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Greek

\newcommand{\balp}{\boldsymbol{\alpha}}
\newcommand{\bbet}{\boldsymbol{\beta}}
\newcommand{\bet}{\boldsymbol{\eta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

%Latin

\newcommand{\bA}{\textbf{A}}
\newcommand{\bD}{\textbf{B}}
\newcommand{\bc}{\textbf{c}}
\newcommand{\bC}{\textbf{C}}
\newcommand{\be}{\textbf{e}}
\newcommand{\bof}{\textbf{f}}
\newcommand{\boof}{\textbf{f}}
\newcommand{\booF}{\textbf{F}}
\newcommand{\boF}{\textbf{F}(\textbf{V})}
\newcommand{\boFU}{\textbf{F}(\textbf{U})}
\newcommand{\boFt}{\textbf{F}(\textbf{t})}
\newcommand{\bFg}{\textbf{F}_{\mathcal{G}}(\bV)}
\newcommand{\bFm}{\textbf{F}_{\mathcal{M}}(\bV)}
\newcommand{\bg}{\textbf{g}}
\newcommand{\bG}{\textbf{G}}
\newcommand{\bGt}{\textbf{G}(\textbf{t})}
\newcommand{\bh}{\textbf{h}}
\newcommand{\bH}{\textbf{H}}
\newcommand{\bHg}{\til{\bH}_{\mathcal{G}}(\bV,t)}
\newcommand{\bHm}{\til{\bH}_{\mathcal{M}}(\bV,t)}
\newcommand{\bI}{\textbf{I}}
\newcommand{\bk}{\textbf{k}}
\newcommand{\bM}{\textbf{M}}
\newcommand{\bP}{\textbf{P}}
\newcommand{\bp}{\textbf{p}}
\newcommand{\bq}{\textbf{q}}
\newcommand{\bQ}{\textbf{Q}}
\newcommand{\br}{\textbf{r}}
\newcommand{\bR}{\textbf{R}}
\newcommand{\bS}{\textbf{S}}
\newcommand{\bu}{\textbf{u}}
\newcommand{\bU}{\textbf{U}}
\newcommand{\bv}{\textbf{v}}
\newcommand{\bV}{\textbf{V}}
\newcommand{\bw}{\textbf{w}}
\newcommand{\bW}{\textbf{W}}

%%%%%%%%%%%%%%%%% letters with hats and tildes %%%%%%%%%%%%%%%%%

\newcommand{\til}{\tilde}
\newcommand{\bDh}{\hat{\textbf{D}}}
\newcommand{\Bh}{\hat{\partial}}
\newcommand{\hh}{\hat{\textbf{h}}}
\newcommand{\bHt}{\tilde{\textbf{H}}(\textbf{V},t)}
\newcommand{\tH}{\tilde{\textbf{H}}}
\newcommand{\bht}{\tilde{\textbf{h}}}
\newcommand{\btr}{\tilde{\textbf{r}}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tr}{\tilde{r}}
\newcommand{\tbr}{\tilde{\textbf{r}}}
\newcommand{\ttim}{\tilde{t}}
\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tth}{\tilde{\theta}}

%%%%%%%%%%%%%%%%% Derivatives %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\deriv}[2]{\frac{\dd #1}{\dd #2}}

%ODE's

\newcommand{\odcxot}{\frac{\dd{\bc_{x0}}}{\dd{t}}}
\newcommand{\odcyot}{\frac{\dd{\bc_{y0}}}{\dd{t}}}
\newcommand{\odcot}{\frac{\dd{\bc_0}}{\dd{t}}}
\newcommand{\odomt}{\frac{\dd{\omega}}{\dd{t}}}
\newcommand{\odRt}{\frac{\dd{R}}{\dd{t}}}
\newcommand{\odbRt}{\frac{\dd{\bR}}{\dd{t}}}
\newcommand{\odTt}{\frac{\dd{\dT}}{\dd{t}}}
\newcommand{\odTht}{\frac{\dd{\Theta}}{\dd{t}}}
\newcommand{\odThot}{\frac{\dd{\Theta_0}}{\dd{t}}}
\newcommand{\odThonet}{\frac{\dd{\Theta_1}}{\dd{t}}}
\newcommand{\odbut}{\frac{\dd{\bu}}{\dd{t}}}
\newcommand{\odbUt}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odut}{\frac{\dd{\bU}}{\dd{t}}}
\newcommand{\odbvt}{\frac{\dd{\bv}}{\dd{t}}}
\newcommand{\odbVt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbVot}{\frac{\dd{\bV_0}}{\dd{t}}}
\newcommand{\odbVpt}{\frac{\dd{\bV_1}}{\dd{t}}}
\newcommand{\odvt}{\frac{\dd{\bV}}{\dd{t}}}
\newcommand{\odbvpit}{\frac{\dd{\bv}_{pi}}{\dd{t}}}
\newcommand{\odbVpit}{\frac{\dd{\bV}_{1pi}}{\dd{t}}}
\newcommand{\odbwt}{\frac{\dd{\bw}}{\dd{t}}}
\newcommand{\odbWt}{\frac{\dd{\bW}}{\dd{t}}}
\newcommand{\odXt}{\frac{\dd{X}}{\dd{t}}}
\newcommand{\odYt}{\frac{\dd{Y}}{\dd{t}}}

%PDE's - wrt x

\newcommand{\pdbvx}{\frac{\partial{\textbf{v}}}{\partial{x}}}
\newcommand{\pdbux}{\frac{\partial{\textbf{u}}}{\partial{x}}}
\newcommand{\pdux}{\frac{\partial{u}}{\partial{x}}}
\newcommand{\pdvx}{\frac{\partial{v}}{\partial{x}}}
\newcommand{\pdvxk}{\frac{\partial{v^{(i)}_k}}{\partial{x}}}
\newcommand{\pduox}{\frac{\partial{\textbf{u}_0}}{\partial{x}}}
\newcommand{\pdvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbvox}{\frac{\partial{\textbf{v}_0}}{\partial{x}}}
\newcommand{\pdbtvox}{\frac{\partial{\til{\textbf{v}}_0}}{\partial{x}}}
\newcommand{\pdvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{x}}}}
\newcommand{\pdbvotx}{\frac{\partial{\textbf{v}_0}}{\partial{\til{x}}}}
\newcommand{\pdvoxx}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}^2}}
\newcommand{\pdtrtx}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{x}}}}
\newcommand{\pdtthtx}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{x}}}}
\newcommand{\pdtxx}{\frac{\partial{\tilde{x}}}{\partial{x}}}
\newcommand{\pdtyx}{\frac{\partial{\tilde{y}}}{\partial{x}}}
\newcommand{\pdax}{\frac{\partial{\alpha}}{\partial{x}}}

%PDE's - wrt y

\newcommand{\pdbvy}{\frac{\partial{\textbf{v}}}{\partial{y}}}
\newcommand{\pduoy}{\frac{\partial{\textbf{u}_0}}{\partial{y}}}
\newcommand{\pdvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoy}{\frac{\partial{\textbf{v}_0}}{\partial{y}}}
\newcommand{\pdbvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\til{y}}}}
\newcommand{\pdvoty}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{y}}}}
\newcommand{\pdvoyy}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}^2}}
\newcommand{\pdtrty}{\frac{\partial{\tilde{\rho}}}{\partial{\tilde{y}}}}
\newcommand{\pdtthty}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{y}}}}
\newcommand{\pdtxy}{\frac{\partial{\tilde{x}}}{\partial{y}}}
\newcommand{\pdtyy}{\frac{\partial{\tilde{y}}}{\partial{y}}}

%PDE's - wrt theta

\newcommand{\pdbvth}{\frac{\partial{\textbf{v}}}{\partial{\theta}}}
\newcommand{\pdvoth}{\frac{\partial{\textbf{v}_0}}{\partial{\theta}}}
\newcommand{\pdvth}{\frac{\partial{\textbf{v}_1}}{\partial{\theta}}}
\newcommand{\pdvotth}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{\theta}}}}
\newcommand{\pdvothth}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}^2}}

%PDE's - wrt t

\newcommand{\pdvvtt}{\frac{\partial{\textbf{v}}_1}{\partial{\tilde{t}}}}
\newcommand{\pduot}{\frac{\partial{\textbf{u}_0}}{\partial{t}}}
\newcommand{\pdbut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvot}{\frac{\partial{\textbf{v}_0}}{\partial{t}}}
\newcommand{\pdvott}{\frac{\partial{\textbf{v}_0}}{\partial{\tilde{t}}}}
\newcommand{\pdtthtt}{\frac{\partial{\tilde{\theta}}}{\partial{\tilde{t}}}}
\newcommand{\pdut}{\frac{\partial{\textbf{u}}}{\partial{t}}}
\newcommand{\pdvt}{\frac{\partial{\textbf{v}}}{\partial{t}}}

%PDE's - wrt u/v/U/V

\newcommand{\pdfa}{\frac{\partial{\textbf{f}}}{\partial{\alpha}}}
\newcommand{\pdfu}{\frac{\partial{\textbf{f}}}{\partial{\bu}}}
\newcommand{\pdfvov}{\frac{\partial{\textbf{f}(\textbf{v}_0)}}{\partial{\textbf{v}}}}
\newcommand{\pdgu}{\frac{\partial{\textbf{g}}}{\partial{\bV}}}

%PDE's mixed

\newcommand{\pdvoxy}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{y}}}
\newcommand{\pdvoxth}{\frac{\partial^2{\textbf{v}_0}}{\partial{x}\partial{\theta}}}
\newcommand{\pdvoyx}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{x}}}
\newcommand{\pdvoyth}{\frac{\partial^2{\textbf{v}_0}}{\partial{y}\partial{\theta}}}
\newcommand{\pdvothx}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{x}}}
\newcommand{\pdvothy}{\frac{\partial^2{\textbf{v}_0}}{\partial{\theta}\partial{y}}}

